Unpacking Reward Shaping: Understanding the Benefits of Reward Engineering on Sample Complexity

Reinforcement learning provides an automated framework for learning behaviors from high-level reward specifications, but in practice the choice of reward function can be crucial for good results -- while in principle the reward only needs to specify what the task is, in reality practitioners often need to design more detailed rewards that provide the agent with some hints about how the task should be completed. The idea of this type of ``reward-shaping'' has been often discussed in the literature, and is often a critical part of practical applications, but there is relatively little formal characterization of how the choice of reward shaping can yield benefits in sample complexity. In this work, we build on the framework of novelty-based exploration to provide a simple scheme for incorporating shaped rewards into RL along with an analysis tool to show that particular choices of reward shaping provably improve sample efficiency. We characterize the class of problems where these gains are expected to be significant and show how this can be connected to practical algorithms in the literature. We confirm that these results hold in practice in an experimental evaluation, providing an insight into the mechanisms through which reward shaping can significantly improve the complexity of reinforcement learning while retaining asymptotic performance.

==> texs/DEPRECATED_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) in its most general form presents a very difficult optimization problem: when there are no constraints on the reward function or dynamics, a learning algorithm may need to exhaustively explore the entire state space to discover high-reward regions. Na\"{i}ve algorithms that rely entirely on random exploration are known to be exponentially expensive, and much of the theoretical work on efficient RL algorithms has focused smarter exploration strategies that aim to more efficiently cover state space, typically in time polynomial in the state space cardinality~\citep{azar2017minimax,jin2018q,zhang2020almost,li2021breaking}. Much of this work is based on upper confidence bound (UCB) principles and prescribes some sort of exploration bonus to prioritize exploration of rarely visited regions. Analogous strategies have also been employed in a number of practical RL algorithms~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration,houthooft2016vime,pathak2017curiosity,vezhnevets2017feudal,VanSeijen2017Hybrid,Raileanu2020RIDE:}. However, perhaps surprisingly, much of the empirical work on reinforcement learning does not make use of explicit exploration bonuses or other dedicated exploration strategies, despite numerous theoretical results showing them to be essential to attain polynomial sample complexity, and despite the existence of numerous practically applicable methods. Instead, practitioners often incorporate prior knowledge of each task into designing or shaping the reward function~\citep{ng1999policy,vinyals2019grandmaster,andrychowicz2020learning,berner2019dota,ye2020towards,zhai2022computational}, preferring this heuristic approach over the more principled exploration strategies. These shaped rewards are not just an implementation detail to make optimization more stable or efficient, but often make the difference between success and complete failure. Why is reward shaping often preferred in practice over dedicated exploration methods?

A likely answer to this question lies in the fact that even the best general-purpose exploration strategies still require visiting every state in the MDP at least once in the worst case. This is of course unavoidable without further assumptions: without any knowledge of where high-reward states are, the agent has no choice but to try visiting all of them. However, in practice, sample complexity that is polynomial in the size of the entire state space might \emph{still} not be practical, and hence prior knowledge in the form of reward shaping is required to render such tasks tractable for RL. Intuitively, this reward shaping provides guidance  during exploration and  prevents an RL agent from doing  uninformed, state covering exploration. Perhaps surprisingly, despite the widespread popularity of reward shaping in RL applications, the analysis of reward shaping has remained limited to proving policy invariance~\citep{ng1999policy} or empirical observations. In this work, we take a step towards studying the effect of reward shaping on the efficiency of RL algorithms, by asking the following question:
%%SL: rewrite the above
%Reinforcement learning (RL) methods aim to learn policies that maximize the overall expected cumulative reward via interaction with an unknown environments~\citep{sutton2018reinforcement}. Many recent works~\citep{azar2017minimax,jin2018q,zhang2020almost,li2021breaking} adopt the Markov decision processes (MDPs) as a theoretical framework and uses regret to quantify the performance in finite horizon, where the regret represents the gap between the accumulative reward received by the learned policy and the optimal policy, using the Upper Confidence Bound (UCB) algorithm~\cite{lattimore2020bandit}. Theoretical analysis of exploration bonus in the aforementioned literature indeed inspires the practical community. For example, some practical works have proposed to add bonuses~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration} or intrinsic rewards~\citep{houthooft2016vime,pathak2017curiosity,vezhnevets2017feudal,VanSeijen2017Hybrid,Raileanu2020RIDE:} to encourage explorations. However, one main practical challenge of applying exploration bonus is the daunting complexity incurred by the entire state space. To resolve such computational challenge, practitioners often incorporate prior knowledge of each task into designing or shaping the reward function~\citep{ng1999policy,andrychowicz2017hindsight,vinyals2019grandmaster,andrychowicz2020learning,berner2019dota,ye2020towards,zhai2022computational}. This is not just an implementation detail to make optimization more stable or efficient, but often makes the difference between success and complete failure on various domains, as evidenced by [cite, cite]. Many large scale successes of practical RL algorithms leverage significant domain knowledge to construct the reward function for different tasks, as shown in Table []. Intuitively this reward shaping provides guidance  during exploration and  prevents an RL agent from doing  uninformed, state covering exploration. However, to the best of our knowledge, the analysis of reward shaping has remained limited to proving policy invariance~\citep{ng1999policy} or empirical observations. In this work, we take a first step towards studying the effect of reward shaping on the efficiency of RL algorithms, by asking the following question:
\begin{center}
    \emph{Can we theoretically justify the complexity benefits of reward shaping with domain knowledge?}
\end{center}
%%SZ.5.18: edited, how about the new one?

%%SL.5.14: It's great to pose the question like this, but maybe we can state this much more briefly? The phrasing above kind of seems a bit roundabout
% For example, the UCBVI algorithm~\citep{azar2017minimax} achieves the regret of $\wt{O}(\sqrt{H^2SAT}+H^4S^2A)$; the UCB-Q-H and UCB-Q-B~\citep{jin2018q} achieve regret of $\wt{O}(\sqrt{H^4SAT}),\wt{O}(\sqrt{H^3SAT}+\sqrt{H^9S^3A^3})$ respectively; the UCB-Q-Advantage~\citep{zhang2020almost} achieves regret of $\wt{O}(\sqrt{H^2SAT}+H^8S^2A^{3/2}T^{1/4})$; and the Q-EarlySettled-Advantage~\citep{li2021breaking} achieves regret of $\wt{O}(\sqrt{H^2SAT}+H^6SA)$, where $H,S,A,T$ are the number of horizons (in episodic finite-horizon), states, actions, and steps (or sample complexity in some other literature). 
%%SL.5.14: Perhaps one way I might suggest to tweak the above paragraph is to borrow some of the phrasing I suggested in the big comment at the end of the abstract, to talk about how in the theory literature, the main way that people go from exp-time to poly-time is by using bonuses. At the same time, I would not recommend to go quite so deep into "related work" in the intro, just summarize it a cursory level and leave the deeper dive for the related work section, otherwise there are too many speedbumps on the way to getting the main message across to the reader.

%% SZ: Thanks for the suggestion, edited!


% The improvements in the regret bounds in the aforementioned literature provide insights into both the theoretical and practical community. From a theoretical perspective, the improvement in these regret bounds are approaching the fundamental lower bound $\Omega(\sqrt{H^2SAT})$ suggested by~\citet{jin2018q,domingues2021episodic}. Practically, the exploration bonus in the UCB type of regret analysis inspires the practical community as many practical works have proposed to add bonuses~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration} or intrinsic rewards~\citep{houthooft2016vime,pathak2017curiosity,vezhnevets2017feudal,VanSeijen2017Hybrid,Raileanu2020RIDE:} to encourage explorations. 

% However, these regret bounds with a dependency on the entire space $S$ are less informative to practice since the state space are either discrete and enormous~\citep{mnih2013playing,mnih2015human,silver2016mastering,silver2017mastering} or continuous~\citep{brockman2016openai,berner2019dota,ye2020towards,tunyasuvunakool2020dm_control}. 

%%SL.5.14: I think this might be barking up the wrong tree. We don't need to convince the reader that exploration bonuses are bad or somehow lacking, it's better to start by convincing the reader that reward shaping is worth analyzing. If indeed we are able to show that our results are significantly better than the best results for bonuses, then we can add some discussion of that too, but later in the intro, kind of like "in the process we show that good reward shaping can actually lead to significantly more favorable sample complexity bounds than uninformed exploration bonuses, which perhaps provides a partial explanation for why such approaches are often preferred in practice over the more principled exploration strategies that can handle arbitrary sparse rewards" (basically, phrase the improvement over bonuses as an added bonuses (heh) rather than the main goal of the paper). The reason to do it this way is to avoid "picking a fight" -- you want to get the reader on your side early, and since the people who will be deciding on whether or not the paper should be accepted will largely be the people that wrote these prior papers, it's good for them to view this work as complementary rather than hostile to their papers.
%%SZ.5.17: Thanks for the suggestion, will update the story accordingly.


%%SL.5.14: I think we need to better motivate this decaying thing. The incongruence between what came before and this paragraph is that we are doing a little bit more than just analyzing *existing* reward shaping, but we are actually proposing a slightly new approach to do reward shaping "right". Maybe we need to tweak some of the motivation to account for this.
We propose a novel regret analysis framework to approach this problem. In our framework, we assume domain knowledge of a reward shaping term $\Vtilde$, that is added as a decaying bonus to the true reward function (as in [cite, cite]). The reward shaping term $\Vtilde$ is not required to be \emph{optimal} and in our analysis is assumed to be a bounded approximation of the optimal value function $\Vstar$. In particular, our analysis assumes that $\Vtilde \leq \Vstar \leq \beta \Vtilde$ where $\beta \geq 1$ and $\Vstar$ is the optimal value function, essentially saying that the optimal value function is always sandwiched by a multiplicative factor of the reward shaping $\Vtilde$. \simon{perhaps aldo or abhishek can help me check whether the next 2 sentences are reasonable} In addition, our formulation is also adaptive to environments containing suboptimal paths that are not visited by the optimal policy. With the bounded assumption on $\Vtilde$, we show that we are able to reduce complexity by [] by simply adding a $\frac{\Vtilde}{N(s, a)}$ term to the reward function and performing simple projected value iteration avoids exploring suboptimal paths effectively. The key pieces of intuition in being able to do this are: 
% In particular, our analysis assumes that $\Vtilde$ is ``sandwiched" % by constant multiplicative factors of the optimal value function $\Vstar$, above and below. 
%%SZ.5.18: I have one alternative, but my suggustion may not be very helpful to practical reward shaper: "In particular, our analysis assumes that $\Vtilde$ is upper bounded $\alpha\Vstar$ by and lower bounded by $\beta\Vstar$, where $\alpha,\beta$ are two multiplicative constants and $\Vstar$ is the optimal value function."
%%SL.5.14: This "sandwiching" thing is a bit hard to parse, I wonder if we can adjust the phrasing here to somehow give the reader a better intuitive understand of what this assumption really means? E.g., try to relate it to things one might expect reward shapers to actually be able to do in practice.

\aldo{Rework these:}
\begin{enumerate}
    \item The knowledge of the sandwich condition of $\Vtilde$ and $\Vstar$ allows us to truncate confidence intervals to prevent ``over-optimism". 
    %%SL.5.14: "knowledge of sandwiching" sounds really strange...
    \item The projection of the value function during value iteration allows us to prune out large parts of the state space via branch and bound since they hardly affect the value function. 
    \item The knowledge of the sandwich term allows us to sharpen the worst case $\epsilon$-net bounds over \emph{all} possible value functions to simply those within bounded range. 
    %%SL.5.14: It's a bit hard to understand what this third point really means
\end{enumerate}

% \aldo{Make sure we cite ~\cite{azar2017minimax} somewhere}
%SZ: \cite{azar2017minimax} is cited in the second sentence of the intro

In doing so, we characterize how reward shaping can provably improve sample efficiency.
%%SL.5.14: maybe be more concrete eg how it can make it polynomial? or better than bonuses? or just better than exponential?
We show that the ``quality" of the provided shaping can significantly affect the sample efficiency of reinforcement learning, but guarantees that the optimal policy remains unchanged
%%SL.5.14: super important caveat here -- only if we use our proposed decaying! not for any arbitrary reward shaping
at convergence. We show that these theoretical insights hold in practice with empirical evaluations in a family of maze navigation problems.

% 1) 
% g; 2) Skip value iteration for certain states which have small enough $\Vtilde$ 3) Skip exploration for certain actions at states which we can branch and bound by forming a $\Qhat$ bound. \simon{same as before, need to rephrase our contributions after the theoretical parts are approximately finalized.}

% satisfies the ``sandwich'' property \simon{need to rephrase the assumptions after the theoretical parts are approximately finalized}. 



% \subsection{Our Results}


\section{Related Work}
\paragraph{Regret Analysis in Finite Horizon Episodic Tabular MDPs}
Recent research on regret analysis has studied on these two types of methods, the model-based methods and model-free methods. Model-based methods~\citep{jaksch2010near,agrawal2017posterior,azar2017minimax,fruit2018efficient,efroni2019tight,pacchiano2021towards} first learn a model from previous experience and use the learned model for future decision making. In contrast, model-free~\citep{jin2018q,bai2019provably,zhang2020almost,yang2021q,menard2021ucb,li2021breaking} aims at learning the value function without the model estimation stage and use the learned value function for decision making. \simon{will need to rephrase the next two sentences after finalizing the theoretical results.} Our analysis lies in the model-based framework and is similar to the setting of~\citep{azar2017minimax} but with additional assumptions on the knowledge of some truncated intervals containing $\Vstar$. The main difference between our results and the aforementioned works is that, the truncated interval assumption can reduce the state dependency $S$ to the smaller truncated states $\bar{S}$, which is more practical. 

\paragraph{Regret Analysis with Linear Function Approximation}
A recent line of literature has investigated the linear function approximation setting by assuming the transition kernels or the value functions can be represented by $d$-dimensional linear features~\citep{jin2020provably,zanette2020frequentist,ayoub2020model,zhou2021provably,cai2020provably,yang2020reinforcement,yang2019sample,wang2019optimism}. With the aforementioned linear assumptions, the regret analysis will only depend on the ambient dimension $d$, instead of $S,A$ in the tabular setting~\citep{wang2019optimism,yang2020reinforcement,cai2020provably,zhou2021provably,ayoub2020model,zanette2019tighter,jin2020provably}, which largely alleviate the complexity. A followup work~\citep{yang2020function} generalized the linear function assumption to general function class and provides a regret bound that only depends on the intrinsic complexity of the function class $\mc F$. \simon{will need to rephrase the following sentences after finalizing the theoretical results}. Our work is related to the function approximation literature in the sense we also assume some prior knowledge of the value functions. However, instead of assuming (generalized) linear features, we assume knowledge of some confidence intervals of the true value functions, which leads to different analysis techniques from the previous function approximation literature.


\paragraph{Practical Reward Design and Reward Shaping}
\citet{ng1999policy} proposed a potential-based shaping function $F$ and showed that the optimal policy under reward function $F+r$ is the same as the optimal policy under original reward function $r$ when the other components in the MDP remains the same. In the practical community, the reward design varies from task to task for different purposes. To achieve super-human performance in some large-scale practical RL tasks, AlphaGo adopts~\citep{silver2016mastering,silver2017mastering} the na\"ive +1 and -1 terminal rewards; while in some other tasks~\citep{berner2019dota,ye2020towards}, the reward functions are heavily handcrafted based on prior knowledge. Practical reward design has also been studied in the goal-conditioned RL~\citep{kaelbling1993learning,andrychowicz2017hindsight,fu2018variational,pong2018temporal,warde2018unsupervised,ghosh2021learning,pong2019skew,eysenbach2020rewriting,eysenbach2021clearning,fujita2020distributed,chebotar2021actionable,zhai2022computational}. Another line of literature also applies count-based reward shaping or intrinsic rewards to encourage explorations~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration,houthooft2016vime,pathak2017curiosity,vezhnevets2017feudal,VanSeijen2017Hybrid,Raileanu2020RIDE:,li2021mural}. \simon{same as before, need to rephrase the following sentences after finalizing the theoretical parts}. Our theoretical analysis is closely connected to the exploration bonus literature~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration} and could potentially shed light on practical count-based exploration algorithms with theoretical guarantees. However, unlike most exploration methods and analyses our analysis analyzes the case  where domain knowledge is available through a ``shaped reward"  function, which can be used to  significantly direct exploration. This is of significant practical relevance since most  practitioners do leverage significant reward shaping, and a deeper theoretical understanding provides insight on what types of reward shaping should be used and how much benefit can be expected. Moreover, our simple algorithm for incorporating (potentially suboptimal) reward shaping provides a  simple way to get the benefit of reward shaping without requiring the shaping functions to be ``potential-based" or optimal. Our results show smoooth degradation to count baseed exploration as shaping becomes more and more uninformative, ensuring asymptotic performance is maintained. 



==> texs/discussion.tex <==
\vspace{-0.5em}
\section{Discussion} 
\label{sec:discussion}
\vspace{-1em}
In this work, we take a step towards formally analyzing the benefits of reward shaping, proving that effective reward shaping can lead to more efficient learning than uninformed exploration strategies. In our analysis, we study an algorithm that incorporates reward shaping into a modified version of UCBVI, using it to modify bonuses and value function projection. Our analysis shows that incorporating shaped rewards allows for pruning significant parts of the state space and sharpening of optimism in a task directed way. This reduces the dependence of the regret bound on the state space size and on the horizon, depending on the quality of the shaping term and parameters of the MDP. This shows how reward shaping can direct exploration and provide significant sample complexity benefits while retaining asymptotic performance. We hope that this work is a step towards moving sample complexity analysis away from being reward agnostic to actually considering reward shaping more formally in analysis. As for future directions, we would also like to study a much broader class of reward shaping and more generic ways to incorporate reward shaping.

==> texs/experimental_details.tex <==
\section{Experimental Details}
\label{sec:exp_details}
We conducted experiments building on the UCBVI framework outlined in ~\cite{azar2017minimax}. Specifically, we used the bonus 1 formulation from Algorithm [] in ~\cite{azar2017minimax}, with the bonus specifically being $\frac{C}{\sqrt{N(s,a)}}$ as the base UCBVI implementation. Our implementation is based on the open source implementation by Ian Osband ~\url{https://github.com/iosband/TabulaRL}, and open source code is attached. 

The implementations of UCBVI-BS replaces this bonus by $\frac{C.\Vtilde}{\sqrt{N(s,a)}}$.  In our implementation we chose the scaling to be $0.1$ with a hyperparameter sweep. The $\Vtilde$ was chosen by scaling the optimal value function $\Vstar$ by factors chosen between $1 + \beta$ and $1 - \beta$,  with $beta$ as $0.2, 0.5, 0.9$ (as described in the experimental section). 

The environments themselves are open gridworlds of size $8$, a corridor of size $10x10$ and the double corridor has size $10x20$. The reward is $0$ everywhere except the goal location.  Every experiment is averaged over 3 random seeds. 

\section{Supporting Algorithms}
\begin{small}
\begin{algorithm}[!h]
  \caption{UCBVI}\label{algo:UCBVI}
  \begin{algorithmic}[1]
    \State \textbf{Input} reward function $r$ (assumed to be known), confidence parameters 
      \State \textbf{for} {$t=1,...,T$}
        \State \qquad Compute $\wh{P}_t$ using all previous empirical transition data as $\wh{\bb P}_t(s^\prime|s,a) := \frac{N_h^t(s,a,s^\prime)}{N_h^t(s,a)},\;\forall h,s,a,s^\prime$.
        \State \qquad Compute reward bonus $b_h^t(s,a)=2H\sqrt{\ln(SAHK/\delta)/N_h^t(s,a)}$
        \State \qquad Run Value-Iteration on $\{\wh{\bb P}_t,r+b_h^t\}_{h=0}^{H-1}$.  
        \State \qquad Set $\pi_t$ as the returned policy of VI.
      \State \textbf{End for }
  \end{algorithmic}
\end{algorithm}
\end{small}

\section{Intuition for $\pseudosub_\Delta$ and $\pathpseudosub_\Delta$}
Here we provide some intuition for the concepts of $\pseudosub_\Delta$ and $\pathpseudosub_\Delta$ in a deterministic chain environment (actions being left and right with deterministic transitions). The environment has a reward of $1$ at state $0$ and $0$ elsewhere. Discount factor is $0.8$ here, and the $\tilde{V}$ has a sandwich factor $\beta=0.3$. The true optimal value function is shown at the top of Fig.~\ref{fig:pseudo_sub_illustration}. The reward shaping is shown in the middle row of Fig.~\ref{fig:pseudo_sub_illustration}. The concept of pseudosub is shown via the arrows at $(s, a)$ pairs that lie in $\pseudosub_\Delta$ for this particular choice of $\tilde{V}$ and $\Delta$. They basically denote states which are suboptimal with $\Delta$ confidence according to the shaping function $\tilde{V}$. Now given this definition of $\pseudosub_\Delta$, the corresponding $\pathpseudosub_\Delta$ is shown in the last row. These are states that can be eliminated via reward shaping. As we can see, around half of the states can be eliminated this way, making exploration much more directed. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/environments/PseudoSubillustration.png}
    \caption{Illustration of the concepts of $\pseudosub_\Delta$ and $\pathpseudosub_\Delta$}
    \label{fig:pseudo_sub_illustration}
\end{figure}


\section{Results for Corrupted $\tilde{V}$}
We evaluate the behavior of UCBVI-Shaped as we use a corrupted version of $\tilde{V}$ for the shaping. In particular, we do this by constructing the sandwiched value function $\tilde{V}$ as described in our experimental evaluation (in this case with $\beta=1.5$ in the corridor environment) and then adding gaussian noise to corrupt the value function. We experiment with corruptions of $0.$, $0.1$, $0.5$, $1.0$ variance, zero-centered gaussian noise. The resulting regret is seen in Fig []. As expected, the results show that corruption of $\tilde{V}$ hurts the results as more and more corruption happens, but still performs better than without any shaping at all. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/environments/courrupted_Vtilde.png}
    \caption{Illustration of behavior with corrupted shaping functions $\tilde{V}$ with varying levels of corruption}
    \label{fig:my_label}
\end{figure}

==> texs/experiments.tex <==
\section{Numerical Simulations}
\label{sec:experiments}
\vspace{-1em}
To show the practical relevance of our analysis on reward shaping we perform some numerical simulations on a family of maze environments with tabular state-action representations, as shown in Fig.~\ref{fig:envs}. These environments have deterministic dynamics and reward. The reward is $0$ at all states except a goal sink state, which has reward $1$. These simulations are aimed at studying the following questions: \textbf{(1)} Does reward shaping improves sample complexity in these types of maze environments over uninformed UCBVI? \textbf{(2)} What is the relative importance of the bonus reweighting and the $\Vtilde$ projection? \textbf{(3)} How does the ``suboptimality'' of $\Vtilde$ impact the resulting sample complexity? \textbf{(4)} Does introducing decayed shaping actually allow for policy convergence? In these experiments, $\Vtilde$ is constructed by scaling the optimal value function $\Vstar$ by per-state scaling factors sampled independently within the range $\beta$. 
\vspace{-0.5em}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[height=0.4\linewidth]{Figures/environments/Grid8.pdf}
         \caption{Value function of Gridworld}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[height=0.4\linewidth]{Figures/environments/SingleCorridor.pdf}
         \caption{Value function of Single Corridor}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[height=0.4\linewidth]{Figures/environments/DoubleCorridor.pdf}
         \caption{Value function of Double Corridor}
     \end{subfigure}
    \caption{\footnotesize{Environments used for numerical simulations. \textbf{(Left)} Open Gridworld  \textbf{(Middle)} Single corridor, agent starts bottom right has to reach a goal in top left  \textbf{(Right)} Double corridor, agent starts in the middle and has to reach a goal on the left, with many irrelevant states on the right hand side}}
    \label{fig:envs}
    \vspace{-1em}
\end{figure}

\subsection{Does reward shaping help direct exploration over optimism under uncertainty?}
\vspace{-0.5em}
We conducted numerical simulations on tabular environments to understand how reward shaping via UCBVI-Shaped provides benefits over standard UCBVI. Fig.~\ref{fig:comparisons_ablations_ucbvi} shows cumulative regret accumulated with different variants of UCBVI-Shaped (with both projection and bonus scaling), UCBVI-Shaped-P (with only projection),  UCBVI-Shaped-BS (with only bonus scaling), UCBVI (standard UCBVI without shaping, as described in ~\cite{azar2017minimax}). This is benchmarked across the three environments described in Fig.~\ref{fig:envs}, with various levels of imperfect shaping applied by varying $\beta = \{1.5, 1.9\}$. As seen from Fig.~\ref{fig:comparisons_ablations_ucbvi}, across all environments UCBVI-shaped with projection and bonus scaling performs most favorably, followed typically by UCBVI-Shaped-P, followed by UCBVI-Shaped-BS and UCBVI, suggesting that reward shaping can significantly help with learning efficiency.

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    % \begin{subfigure}[b]{0.3\textwidth}
    %      \centering
    %      \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/grid8_UCBVIvsRest_shaping0.png}
    %      \caption{Open Gridworld, $\beta = 1.0$}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.3\textwidth}
    %      \centering
    %      \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/corridor_UCBVIvsRest_shaping0.png}
    %      \caption{Single Corridor, $\beta = 1.0$}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.3\textwidth}
    %      \centering
    %     \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/doublecorridor_UCBVIvsRest_shaping0.png}
    %      \caption{Double Corridor, $\beta = 1.0$}
    %  \end{subfigure} \\
     
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/grid8_UCBVIvsRest_shaping05.png}
         \caption{Open Gridworld, $\beta = 1.5$}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/corridor_UCBVIvsRest_shaping05.png}
         \caption{Single Corridor, $\beta = 1.5$}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/doublecorridor_UCBVIvsRest_shaping05.png}
         \caption{Double Corridor, $\beta = 1.5$}
     \end{subfigure} \\
     
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/grid8_UCBVIvsRest_shaping09.png}
         \caption{Open Gridworld, $\beta = 1.9$}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/corridor_UCBVIvsRest_shaping09.png}
         \caption{Single Corridor, $\beta = 1.9$}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includegraphics[width=\linewidth]{Figures/Experiment0_UCBVI_vs_others/doublecorridor_UCBVIvsRest_shaping09.png}
         \caption{Double Corridor, $\beta = 1.9$}
     \end{subfigure}
    \caption{Cumulative regret for learning in various environments with varying amounts of shaping, as compared with UCBVI, and ablations UCBVI-Shaped-BS (no projection) and UCBVI-Shaped-P (no bonus scaling)}
    \label{fig:comparisons_ablations_ucbvi}
    % \vspace{-2em}
\end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.32\linewidth]{Figures/Experiment0_UCBVI_vs_others/grid8_UCBVIvsRest_shaping05.png}
%     \includegraphics[width=0.32\linewidth]{Figures/Experiment0_UCBVI_vs_others/corridor_UCBVIvsRest_shaping05.png}
%     \includegraphics[width=0.32\linewidth]{Figures/Experiment0_UCBVI_vs_others/doublecorridor_UCBVIvsRest_shaping05.png}
%     \caption{Cumulative regret for learning in various environments with perfect reward shaping, with $\beta = 1.5$}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.32\linewidth]{Figures/Experiment0_UCBVI_vs_others/grid8_UCBVIvsRest_shaping09.png}
%     \includegraphics[width=0.32\linewidth]{Figures/Experiment0_UCBVI_vs_others/corridor_UCBVIvsRest_shaping09.png}
%     \includegraphics[width=0.32\linewidth]{Figures/Experiment0_UCBVI_vs_others/doublecorridor_UCBVIvsRest_shaping09.png}
%     \caption{Cumulative regret for learning in various environments with significantly imperfect reward shaping, with $\beta = 1.9$}
%     \label{fig:my_label}
% \end{figure}

\vspace{-1em}
\subsection{How does the effectiveness of reward shaping vary across environments?}
\vspace{-0.5em}
We conducted some numerical simulations across environments to understand how the nature of the environment itself affects the sample complexity of learning with shaping via UCBVI-Shaped. As shown in Fig.~\ref{fig:viz_across_envs}, we see that UCBVI shaped can be very effective in environments with many irrelevant sub-optimal paths like the double corridor environment in Fig.~\ref{fig:envs}, but is relatively less effective in environments where all exploration is directed the same way such as the single corridor. Even incorrect but optimistic shaping will provide guidance towards the goal, making UCBVI relatively less dominant in the single corridor environment as compared to double corridor. This suggests that in environments where ruling out an entire part of the exploration space is easy from the shaping, we can expect to see larger benefits, as in double corridor. 


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{Figures/heatmaps/single_corridor.png}
         \caption{Heatmap of intermediate visitations of UCBVI on single corridor (no shaping)}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{Figures/heatmaps/single_corridor_UCBVIshaped.png}
         \caption{Heatmap of intermediate visitations of UCBVI-Shaped on single corridor}
     \end{subfigure}
      \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Experiment0_UCBVI_vs_others/corridor_UCBVIvsRest_shaping02.png}
         \caption{Learning progress of UCBVI-Shaped compared to UCBVI on single corridor}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/heatmaps/double_corridor.png}
         \caption{Heatmap of intermediate visitations of UCBVI on double corridor (no shaping)}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/heatmaps/double_corridor_UCBVIshaped.png}
         \caption{Heatmap of intermediate visitations of UCBVI-Shaped on double corridor}
     \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Experiment0_UCBVI_vs_others/doublecorridor_UCBVIvsRest_shaping02.png}
         \caption{Learning progress of UCBVI-Shaped compared to UCBVI on double corridor}
     \end{subfigure}
        \caption{Visualization of how different environments are affected by reward shaping differently. (Left) intermediate visitations (Right) learning progress of UCBVI vs UCBVI-Shaped. The single corridor environment on the top sees much smaller gains for UCBVI-Shaped compared to double corridor environment.}
        \label{fig:viz_across_envs}
        \vspace{-0.5em}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\linewidth]{Figures/heatmaps/single_corridor.png}
%     \caption{Cumulative regret for learning in []}
%     \label{fig:my_label}
% \end{figure}

\subsection{How does the suboptimality of reward shaping affect learning?}
% \vspace{-0.5em}


\begin{wrapfigure}{r}{0.7\linewidth}
    \vspace{-1em}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{Figures/Experiment1_imperfect_shaping_comparison/corridor_UCBVIvsRest_allcomparisonspng.png}
        \caption{Single Corridor}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{Figures/Experiment1_imperfect_shaping_comparison/doublecorridor_UCBVIvsRest_allcomparisons.png}
        \caption{Double Corridor}
    \end{subfigure}
    \caption{Effect of suboptimality of reward shaping on the performance of UCBVI-Shaped. While $\beta=1.2, 1.5$ don't make much of a difference, very large $\beta$ leads to performance degradation}
    \label{fig:suboptimal-shaping}
    \vspace{-1em}
\end{wrapfigure}


We next compared how different levels of suboptimality of the $\beta$ sandwich term in the reward shaping affect cumulative regret across environments. As shown in Fig.~\ref{fig:suboptimal-shaping}, we see that for environments with open paths (Fig.~\ref{fig:suboptimal-shaping} (a), the shaping degradation has minimal negative effect until it gets very suboptimal. On the other hand, for corridor and double corridor (Fig.~\ref{fig:suboptimal-shaping} (b), where there are only a few paths to the goal, suboptimal reward shaping along those paths can significantly hamper progress. This suggests that suboptimal reward shaping can hurt learning, but mainly when $\beta$ is quite large and in environments with bottlenecks. \vspace{-0.5em}


\subsection{Does decaying suboptimal reward shaping help over standard shaped rewards?}
\vspace{-0.5em}
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\linewidth]{Figures/Experiment2_decay/compare_decay_nodecay_UCBVI.png}
        \caption{Quantitative comparison of effect of bonus decay}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=0.8\linewidth]{Figures/Experiment2_decay/stuck_UCBVI_nodecay.png}
        \caption{Visualization of non decaying agent getting stuck}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=0.8\linewidth]{Figures/Experiment2_decay/notstuck_UCBVI_shaped_decay.png}
        \caption{Visualization of decaying agent (UCBVI-Shaped) reaching goal}
    \end{subfigure}
    \caption{\footnotesize{Effect of bonus decay on the performance of UCBVI-Shaped vs standard reward shaping under shaping misspecification. As we can see, without decay the agent can stuck in arbitrarily sub-optimal points, whereas with decay the agent easily converges to an optimal solution.}}
    \label{fig:decay}
    \vspace{-1em}
\end{figure}
We ran simulations to understand whether the adaptive decay of $\Vtilde$ by $\frac{1}{\sqrt{N(s, a)}}$ actually provides tangible benefits, specifically when the shaping is suboptimal. We compared UCBVI-Shaped with a variant where $\Vtilde$ is added to the reward linearly, as done in many practical RL implementations. As seen in Fig.~\ref{fig:decay}, with suboptimal shaping, UCBVI-shaped dampens the effect of the suboptimal shaping and succeed, whereas simple addition of shaping leads to the agent becoming trapped. This suggests that not only can reward shaping improve sample efficiency, but incorporating reward shaping via UCBVI-Shaped can mitigate the potential bias from suboptimal shaping. \vspace{-0.5em}
% \subsection{Visualizations of Shaping and Learned Value Functions}

% We next visualize some of the different variants of shaped rewards and the resulting learned value functions over time. We see that with suboptimal rewards, the agent often gets trapped in suboptimal states intermittently but once scaled down by the counts appropriately, reaches the goal and places density at the appropriate target location. [TODO, what does this verify??]
% Some plots of the Vtildes and visitations over time. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\linewidth]{Figures/heatmaps/heatmap_ep12000.png}
%     \caption{Cumulative regret for learning in []}
%     \label{fig:my_label}
% \end{figure}

==> texs/introduction_new.tex <==
\section{Introduction}
\label{sec:intro}
\vspace{-0.5em}
Reinforcement learning (RL) in its most general form presents a very difficult optimization problem: when there are no constraints on the reward function or dynamics, a learning algorithm may need to exhaustively explore the entire state space to discover high-reward regions. Na\"{i}ve algorithms that rely entirely on random exploration are known to be exponentially expensive~\citep{kakade2003sample,agarwal2020pc}, and much of the theoretical work on efficient RL algorithms has focused smarter exploration strategies that aim to more efficiently cover state space, typically in time polynomial in the state space cardinality~\citep{auer2008near,azar2017minimax,jin2018q,zhang2020almost,li2021breaking,pacchiano2020optimism,zanette2019tighter}. Much of this work is based on upper confidence bound (UCB) principles and prescribes some kind of exploration bonus to prioritize exploration of rarely visited regions. Analogous strategies have also been employed in a number of practical RL algorithms~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration,houthooft2016vime,pathak2017curiosity,vezhnevets2017feudal,VanSeijen2017Hybrid,Raileanu2020RIDE:}. However, surprisingly, much of the empirical work on reinforcement learning does not make use of explicit exploration bonuses or other dedicated exploration strategies, despite numerous theoretical results showing them to be essential to attain polynomial sample complexity. Instead, practitioners often incorporate prior knowledge of each task into designing or shaping the reward function~\citep{ng1999policy,silver2016mastering,silver2017mastering,vinyals2019grandmaster,andrychowicz2020learning,berner2019dota,ye2020towards,zhai2022computational}, preferring this heuristic approach over the more principled exploration strategies. At this point, one may wonder why is reward shaping often practically preferable to dedicated exploration?

A likely answer to this question lies in the fact that even the best general-purpose exploration strategies still require visiting every state in the MDP at least once in the worst case. This is of course unavoidable without further assumptions. However, in practice, sample complexity that is polynomial in the size of the entire state space might \emph{still} not be practical, and hence prior knowledge in the form of reward shaping is required to render such tasks tractable for RL. Surprisingly, despite the widespread popularity of reward shaping in RL applications, the analysis of reward shaping has remained limited to proving policy invariance~\citep{ng1999policy} or largely empirical observations, often relegating reward shaping to folk knowledge. In this work, we take a step towards studying the effect of reward shaping on the efficiency of RL algorithms, by asking the following question:\vspace{-0.5em}
\begin{center}
    \emph{Can we theoretically justify the sample complexity benefits that reward shaping from prior domain knowledge can provide for reinforcement learning?}\vspace{-0.5em}
\end{center}
In this work, we aim to provide a set of tools that formally analyze how reward shaping can improve the complexity of tabula-rasa RL and direct better exploration. To perform this analysis, we first propose a simple modification to standard RL algorithms \textemdash ``UCBVI-Shaped'' that incorporates shaped rewards into optimism based exploration. We use this algorithm instantiation to then provide a regret analysis framework that studies how this introduction of shaped rewards can (in certain cases) provide much more directed optimism than uninformed exploration, while maintaining asymptotic performance. 

To approach our analysis, we specifically consider problems where the reward shaping is provided through a term $\Vtilde$, a (potentially suboptimal) approximation of the optimal value function $\Vstar$. In particular, we assume that the shaping $\Vtilde$ is a multiplicatively bounded approximation of the optimal value function $\Vstar$, i.e., $ \Vtilde(s) \leq \Vstar(s) \leq \beta \Vtilde(s), \forall s$, for a finite multiplicative factor $\beta$. This type of shaped reward function $\Vtilde$ can be incorporated into a standard RL algorithm like UCBVI~\citep{azar2017minimax} through two channels - (1) bonus scaling: simply reweighting a standard, decaying count-based bonus $\frac{1}{\sqrt{N_h(s, a)}}$ by the per-state reward shaping and (2) value projection: adaptively projecting learned value functions into ranges of value functions derived from the reward shaping. 

% [TODO: Aldo can you add a little line about the actual analysis result we get here. I'm not sure how theory people write things.]

We show that this relatively simple algorithmic instantiation lends itself to a simple analysis which shows significant complexity benefits with shaping. Intuitively, the key pieces in our complexity analysis of UCBVI-Shaped are two-fold: 1) The multiplicative sandwich condition (via $\beta$) between $\Vtilde$ and $\Vstar$ allows for the bonus scaling to depend on $\beta \Vtilde$ instead of a coarse approximation of $\Vstar$ such as $H$. This allows for a reduction of complexity from a horizon $H$ dependent term to one scaling with $\beta\Vtilde \leq \beta\Vstar$ by allowing for a faster decay of the exploration bonuses while still providing enough optimism; 2) The projection of the value function prevents ``over optimism'' by hastening the convergence of the empirical $\Qhat$ functions during value iteration thus allowing for faster detection of sub-optimal actions. This results in the ability to prune out large parts of the state space, as we will also validate empirically. % resulting in a significant reduction in the $|\Scal|$ factor.

To concretize, the key contribution of this work is mainly to characterize how reward shaping can provably improve sample efficiency by providing gains in both $|\Scal|$ and $H$ dependent terms. We emphasize that while the algorithm itself is well founded and can be a practical choice for practitioners, this paper is mainly about instantiating an analysis framework that allows us to study the sample complexity of learning in a way that is dependent on the specific type of reward shaping.  
We do so by analyzing the gains from reward shaping in two different ways \textemdash bonus scaling and value projection. We show that the ``quality'' (determined by $\beta$) of the provided shaping can significantly affect the sample efficiency of the resulting reinforcement learning algorithm. Finally, we show that these theoretical insights hold in practice with numerical simulation in a family of maze navigation problems. 

\section{Related Work}
\vspace{-0.5em}
\paragraph{Regret Analysis in Finite Horizon Episodic Tabular MDPs}
Recent research on regret analysis has studied both model-based and model-free RL methods. Model-based methods~\citep{jaksch2010near,agrawal2017posterior,azar2017minimax,fruit2018efficient,efroni2019tight,pacchiano2021towards} first learn a model from previous experience and use the learned model for future decision making. In contrast, model-free methods~\citep{jin2018q,bai2019provably,zhang2020almost,yang2021q,menard2021ucb,li2021breaking} aim to learning the value function without the model estimation stage and use the learned value function for decision making. Our analysis lies in the model-based framework and is similar to the setting of~\citep{azar2017minimax} but with additional assumptions on knowing $\Vtilde$ as a multiplicatively bounded approximation of $\Vstar$. The main difference between our results and the aforementioned works is that, the truncated interval assumption can reduce the state dependency $|\Scal|$ to the some smaller ``effective state space'' and reduce horizon dependency. \vspace{-0.5em}

\paragraph{Regret Analysis with Linear Function Approximation}
A recent line of literature has investigated the linear function approximation setting by assuming the transition kernels or the value functions can be represented by $d$-dimensional linear features~\citep{jin2020provably,zanette2020frequentist,ayoub2020model,zhou2021provably,cai2020provably,yang2020reinforcement,yang2019sample,wang2019optimism} or even general function classes~\citep{yang2020function}. With the aforementioned assumptions, the regret analysis will only depend on the ambient dimension $d$ (or other intrinsic complexity measure), instead of $|\Scal|,|\Acal|$ in the tabular setting~\citep{wang2019optimism,yang2020reinforcement,cai2020provably,zhou2021provably,ayoub2020model,zanette2019tighter,jin2020provably}, which could greatly decrease the complexity of learning. Instead of posing structural assumptions on the function class representing the MDP's values or dynamics, we ask the question of whether having approximate knowledge of $\Vstar$ enables efficient learning. \vspace{-0.5em}

%Our work is related to the function approximation literature in the sense we also assume some prior knowledge of the value functions. However, instead of assuming (generalized) linear features, we assume knowledge of $\Vtilde$, which leads to different analysis techniques from the previous function approximation literature. %A followup work~\citep{yang2020function} generalized the linear function assumption to general function class and provides a regret bound that only depends on the intrinsic complexity of the function class $\mc F$. 


\paragraph{Practical Reward Design and Reward Shaping}
\citet{ng1999policy} proposed a potential-based shaping function $F$ that ensures policy invariance under transformation. However, unbiased potential based reward shaping is rarely used in practice. In most applications, heuristic reward design is carefully performed with  potentially biased reward functions. In some large-scale practical RL tasks~\citep{berner2019dota,ye2020towards, yu2019metaworld}, the reward functions are heavily handcrafted based on prior knowledge. Besides reward engineering, a distinct line of work applies uninformed exploration algorithms like count-based reward shaping or intrinsic rewards to encourage greater state visitation~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration,houthooft2016vime,pathak2017curiosity,vezhnevets2017feudal,VanSeijen2017Hybrid,Raileanu2020RIDE:,li2021mural}. Importantly, these methods optimize for the worst case, as they try to cover \emph{all} states since the exact location of the reward is unknown. In contrast, we look at the problem of incorporating domain knowledge via reward shaping into the exploration process. 

%As we will show later, this allows for significant gains over uninformed exploration since large parts of the state space and value function space can be eliminated with the shaping. \vspace{-0.5em}

% \simon{same as before, need to rephrase the following sentences after finalizing the theoretical parts}.


% Our theoretical analysis is closely connected to the exploration bonus literature~\citep{tang2017exploration,stadie2015incentivizing,bellemare2016unifying,burda2018exploration} and could potentially shed light on practical count-based exploration algorithms with theoretical guarantees.

% However, unlike most exploration methods and analyses our analysis analyzes the case  where domain knowledge is available through a ``shaped reward"  function, which can be used to  significantly direct exploration. 
% This is of significant practical relevance since most  practitioners do leverage significant reward shaping, and a deeper theoretical understanding provides insight on what types of reward shaping should be used and how much benefit can be expected. Moreover, our simple algorithm for incorporating (potentially suboptimal) reward shaping provides a  simple way to get the benefit of reward shaping without requiring the shaping functions to be ``potential-based" or optimal. Our results show smoooth degradation to count baseed exploration as shaping becomes more and more uninformative, ensuring asymptotic performance is maintained. 



==> texs/method.tex <==

\section{The UCBVI-Shaped Algorithm}
\label{sec:method}
\vspace{-0.5em}
To perform analysis of reward shaping, we build on the framework of the UCBVI algorithm~\citep{azar2017minimax}. This forms a convenient base algorithm for incorporating shaped rewards in a way that admits faster learning while maintaining asymptotic performance (as we will discuss in Section~\ref{sec:analysis}). Our algorithm, UCBVI-Shaped, is a combination of two changes to the upper confidence bound algorithm - first we modify the bonus scaling to depend on $\Vtilde$ and second, we introduce a projection subroutine into value iteration, that is implemented as a standard clipping operation. 

\begin{small}
\begin{algorithm}[!h]
  \caption{UCBVI - Shaped}\label{algo:UCBVI_shaped}
  \begin{algorithmic}[1]
    \State \textbf{Input} reward function $r$ (assumed to be known), confidence parameters 
      \State \textbf{for} {$t=1,...,T$}
        \State \qquad Compute $\wh{P}_t$ using all previous empirical transition data as $\wh{\bb P}_h^t(s^\prime|s,a) := \frac{N_h^t(s,a,s^\prime)}{N_h^t(s,a)},\;\forall h,s,a,s^\prime$.
        \State \qquad Compute reward bonus \textcolor{blue}{$b_h^t(s, a)$ from Eqn.~\ref{eq::shaped_bonus}} \Comment{\textcolor{blue}{Bonus scaling}}
        \State \qquad Run Value-Iteration with Projection (Algorithm~\ref{algo:ValueIterationProj}).  
        \State \qquad Set $\pi_t$ as the returned policy of VI.
      \State \textbf{End for }
  \end{algorithmic}
\end{algorithm}
\end{small}

As in standard UCBVI, we define $N_h^t(s,a)$ to be the visitation count for the state-action pair $(s,a)$ at iteration $t-1$ for horizon $h$: ${N_h^t(s,a) := \sum_{i=0}^{t-1}\indicator{(s^i_h,a_h^i)=(s,a)}}$. Similarly to $N_h^t(s,a)$, we use $N_h^t(s,a,s^\prime) := \sum_{i=0}^{t-1}\indicator{(s_h^i,a_h^i,s^i_{h+1}) = (s,a,s^\prime)}$ as the visitation count of state-action pair $(s,a)$ and the subsequent state $s^\prime$. We then use $\wh{\bb P}_t(s^\prime|s,a) := \frac{N_h^t(s,a,s^\prime)}{N_h^t(s,a)},\;\forall h,s,a,s^\prime$ to denote the empirical transition kernels at iteration $t$. UCBVI uses value iteration with the empirical transition function $\wh{\bb P}_t$ and a reward function augmented with an exploration bonus, given by $r_h+b_h^t$. This is defined as a dynamic programming procedure that starts at $H$ and then proceeds backward in time to $h=0$, updating according to Algorithm~\ref{algo:UCBVI_shaped} and~\ref{algo:ValueIterationProj}. The key algorithmic changes between UCBVI and UCBVI-Shaped are highlighted in blue - (1) scaling bonus $b_h^t$ by the shaping term $\Vtilde$ and (2) projecting the empirical value function $\wh{V}_h^t(s)$ by an upper bound based on the sandwiched shaping, $\beta\Vtilde(s,a)$. 

% \begin{algorithm}[ht]
%   \caption{UCBVI - Shaped}\label{algo:UCBVI_shaped-main}
%   \begin{algorithmic}[1]
%     \State \textbf{Input} reward function $r$ (assumed to be known), confidence parameters 
%       \State \textbf{for} {$t=1,...,T$}
%         \State \qquad Compute $\wh{P}_t$ using all previous empirical transition data.
%         \State \qquad Compute reward bonus $b_h^t$, $\forall h$.
%         \State \qquad Run Value-Iteration with Projection (Algorithm~\ref{algo:ValueIterationProj}).  
%         \State \qquad Set $\pi_t$ as the returned policy of VI.
%       \State \textbf{End for }
%   \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[ht]
%   \caption{Value Iteration with Projection}\label{algo:ValueIterationProj-main}
%   \begin{algorithmic}[1]
%   \State \textbf{Input} $\Brac{\wh{P}_t,r+b_h^t}_{h=0}^{H-1}$.
%     \State \aldo{I think it would be helpful to keep the formula for Value Iteration.}
%         \State \qquad Run Value Iteration while clipping each $\Vhat^t_h$ above by interval $ \beta\Vtilde_h$. 
%   \end{algorithmic}
% \end{algorithm}


    % \begin{equation}
    %     \label{eq:VI}
    %     \begin{split}
    %         \wh{V}_H^t(s) =&\; 0,\;\forall s,\\
    %         \wh{Q}_h^t(s,a) =&\min\Brac{r_h(s,a)+b_h^t(s,a)+\wh{\bb P}_t(\cdot|s,a)\cdot\wh{V}_{h+1}^t,H},\\
    %         \wh{V}^k_h =& \max_a\wh{Q}_h^t(s,a),\;\pi_h^t(s) = \arg\max_a\wh{Q}_h^t(s,a),\;\forall h,s,a.
    %     \end{split}
    % \end{equation}
% We can now define UCBVI-Shaped in Algorithm~\ref{algo:UCBVI_shaped}.
%%SL.5.18: A few suggestions: (1) highlight differences from UCBVI in red; (2) add a little bit of discussion to provide an intuition for the algorithm, particularly the modified bonus



\begin{small}
\begin{algorithm}[!h]
  \caption{Value Iteration with Projection}\label{algo:ValueIterationProj}
  \begin{algorithmic}[1]
  \State \textbf{Input} $\Brac{\wh{P}_h^t,r+b_h^t}_{h=0}^{H-1}$.
    % \State $\wh{V}_H^t(s) =\; 0,\;\forall s,\wh{Q}_h^t(s,a)$
    %SZ.5.19: I removed $\wh{Q}_h^t(s,a)$ in the above equation as it is not used
    \State $\wh{V}_H^t(s) =\; 0,\;\forall s,\wh{Q}_h^t(s,a)$
    \State \textbf{While} not converged
    \State \qquad $\wh{Q}_h^t(s,a) =  \min\Brac{r_h(s,a)+b_h^t(s,a)+\wh{\bb P}_h^t(\cdot|s,a)\cdot\wh{V}_{h+1}^t,H}$
    \State \qquad $\wh{V}^t_h(s, a) =\textcolor{blue}{\min \Big(}\max_a\wh{Q}_h^t(s,a)\textcolor{blue}{, \beta\Vtilde(s, a)\Big)}$  \Comment{\textcolor{blue}{Value projection}}
    \State $\pi_h^t(s) = \arg\max_a\wh{Q}_h^t(s,a),\;\forall h,s,a.$
    % \State \qquad Run Value Iteration while clipping each $\Vhat^t_h$ above by interval $ \beta\Vtilde_h$. 
  \end{algorithmic}
\end{algorithm}
\end{small}\vspace{-0.5em}
    % \begin{equation}
    %     \label{eq:VI}
    %     \begin{split}
    %         \wh{V}_H^t(s) =&\; 0,\;\forall s,\\
    %         \wh{Q}_h^t(s,a) =&\min\Brac{r_h(s,a)+b_h^t(s,a)+\wh{\bb P}_t(\cdot|s,a)\cdot\wh{V}_{h+1}^t,H},\\
    %         \wh{V}^k_h =& \max_a\wh{Q}_h^t(s,a),\;\pi_h^t(s) = \arg\max_a\wh{Q}_h^t(s,a),\;\forall h,s,a.
    %     \end{split}
    % \end{equation}

==> texs/old_proof_ucbvi.tex <==
\section{Old Proof UCBVI}





\begin{theorem}[Regret Bound of UCBVI (Section 7.2 of \cite{agarwal2019reinforcement})] 
\label{thm::UCBVI}
\aldo{This is wrong ... }

UCBVI achieves the following regret bound:
\begin{equation}
    \mr{Regret} := \bb E\brac{\sum_{k=0}^{K-1}\paren{V^\star(s_0)-V^{\pi^k}(s_0)}}\leq 10 H^2 S \sqrt{AK\cdot \ln\paren{SAH^2K^2}} =\wt{O}\paren{H^2S\sqrt{AK}}
\end{equation}
\end{theorem}
\begin{proof}
\label{proof:UCBVI}
Consider episode $k$ and denote $\mc H_{<k}$ as the history up to the end of episode $k-1$. We consider bounding $V^\star - V^{\pi^k}$. Using the optimism and the simulation lemma, \highlight{$\forall s\in \mc S_e$, we have}
\begin{equation}
    \begin{split}
        &V^\star(s_0) - V^{\pi^k}(s_0) = V_0^\star(s_0) - V_0^{\pi^k}(s_0)\leq \wh{V}_0^k(s_0)-V_0^{\pi^k}(s_0)\highlight{\leq \tilde{V}_0^k(s_0)-V_0^{\pi^k}(s_0)}\\
        \leq &\sum_{h=0}^{H-1}\bb E_{s_h,a_h\sim d_h^{\pi^k}}\brac{b_h^k(s_h,a_h)+\paren{\wh{P}_h^k(\cdot|s_h,a_h)-P^\star(\cdot|s_h,a_h)}\cdot\highlight{\tilde{V}_{h+1}^{\pi^k}}},
    \end{split}
\end{equation}
where the first inequality holds due to the optimism inequality and the second inequality holds due to the simulation lemma. And \highlight{$\forall s\in \bar{\mc S}_e$}, we have 
\highlight{\begin{equation}
    V^\star(s_0) - V^{\pi^k}(s_0)\leq \eps.
\end{equation}}
Let $\mc E_\mr{model}$ denote the event that Corollary \ref{corollary::variance_bonus_domination} and Lemma \ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} hold. We know that $\mc E_\mr{model}$ happens with probability at least $1-2\delta$. Under $\mc E_\mr{model}$ and \highlight{$\forall s\in \mc S_e$}, we can bound $\paren{\wh{P}_h^k(\cdot|s_h,a_h)-P^\star(\cdot|s_h,a_h)}\cdot\highlight{\tilde{V}_{h+1}^{\pi^k}}$ \highlight{using Lemma \ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} by}
\begin{equation}
    \begin{split}
        &\abs{\paren{\wh{P}_h^k(\cdot|s_h,a_h)-P^\star(\cdot|s_h,a_h)}\cdot\highlight{\tilde{V}_{h+1}^{\pi^k}}}\\
        \leq &32 \sqrt{\left( \frac{3\beta^2}{2} - \frac{1}{2}\right) } \cdot \sqrt{ \frac{\highlight{|\mc S_e|} \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\tilde{V}_{h+1}(s') | s,a)  \ln\paren{\frac{ 2\highlight{|\mc S_e|} |\Acal| t}{\delta}\highlight{(1+\beta H\sqrt{|\mc S_e|}/\eps)}} }{ N_t(s,a) }}\\
        &+ \quad \frac{\highlight{26}H\highlight{|\mc S_e|}}{N_t(s,a)}\ln \paren{\frac{ 2 \highlight{|\mc S_e|} |\Acal|t}{\delta}\highlight{(1+2\beta H\sqrt{|\mc S_e|}/\eps)}}.
    \end{split}
\end{equation}
Hence, for the per-episode regret $V^\star(s_0) - V^{\pi^k}(s_0)$ and \highlight{$\forall s_0\in \mc S_e$}, we have
\begin{equation}
    \label{eq:thm_UCBVI_derivation1}
    \begin{split}
        &V^\star(s_0) - V^{\pi^k}(s_0)\\
        \leq&32 \sum_{h=0}^{H-1}\bb E_{s_h,a_h\sim d_h^{\pi^k}}\Bigg\{\sqrt{\left( \frac{3\beta^2}{2} - \frac{1}{2}\right) } \cdot \sqrt{ \frac{\highlight{|\mc S_e|} \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\tilde{V}_{h+1}(s') | s,a)  \ln\paren{\frac{ 2\highlight{|\mc S_e|} |\Acal| t}{\delta}\highlight{(1+\beta H\sqrt{|\mc S_e|}/\eps)}} }{ N_t(s,a) }}\\
        &+ \brac{ \frac{\highlight{26}H\highlight{|\mc S_e|}}{N_t(s,a)}\ln \paren{\frac{ 2 \highlight{|\mc S_e|} |\Acal|t}{\delta}\highlight{(1+2\beta H\sqrt{|\mc S_e|}/\eps)}}}\\
        &+16\sqrt{ \frac{ \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a)  \ln\frac{ 2 \highlight{|\mc S_e|} |\Acal| t}{\delta} }{ N_t(s,a) }} + \frac{12H}{N_t(s,a)}\ln \frac{ 2 \highlight{|\mc S_e|}|\Acal|t}{\delta}\Bigg\}\\
        \overset{(i)}{\leq} & CH\sqrt{\highlight{|\mc S_e|}\ln (\highlight{|\mc S_e|}|\Acal|KH/\delta)}\cdot\bb E\brac{\sum_{h=0}^{H-1}\frac{\highlight{\widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a)}}{\sqrt{N_h^k(s_h^k,a_h^k)}}|\mc H_{<k}},
    \end{split}
\end{equation}
where inequality $(i)$ follows the definition of the bonus \eqref{eq::bonus}. Now if we sum all episodes together and take the failure event into consideration:
\begin{equation}
    \label{eq:thm_UCBVI_derivation2}
    \begin{split}
        &\bb E\brac{\sum_{k=0}^{K-1}V^\star(s_0)-V^{\pi^k}(s_0)}\\
        = &\bb E\brac{\indicator{\mc E_\mr{model}}\paren{\sum_{k=0}^{K-1}V^\star(s_0)-V^{\pi^k}(s_0)}}+\bb E\brac{\indicator{\bar{\mc E}_\mr{model}}\paren{\sum_{k=0}^{K-1}V^\star(s_0)-V^{\pi^k}(s_0)}}\\
        \leq & \bb E\brac{\indicator{\mc E_\mr{model}}\paren{\sum_{k=0}^{K-1}V^\star(s_0)-V^{\pi^k}(s_0)}} + 2\delta KH\\
        \leq & CH\sqrt{\highlight{|\mc S_e|}\ln (\highlight{|\mc S_e|}|\Acal|KH/\delta)}\cdot\bb E\brac{\sum_{h=0}^{H-1}\frac{\highlight{\widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a)}}{\sqrt{N_h^k(s_h^k,a_h^k)}}|\mc H_{<k}}+2\delta KH,
    \end{split}
\end{equation}
where the last inequality follows \eqref{eq:thm_UCBVI_derivation1}. Now we can bound the final term in \eqref{eq:thm_UCBVI_derivation2} using Lemma \ref{lemma:UCBVI_final_bound}:
\begin{equation}
    \bb E\brac{\sum_{k=0}^{K-1}V^\star(s_0)-V^{\pi^k}(s_0)}\leq CH^2\highlight{|\mc S_e|}\sqrt{AK\ln(\highlight{|\mc S_e|}|\Acal|HK/\delta)}+2\delta KH,
\end{equation}
where $C$ is a constant. Set $\delta = 1/KH$, we have 
\begin{equation}
    \bb E\brac{\sum_{k=0}^{K-1}V^\star(s_0)-V^{\pi^k}(s_0)}\leq O(H^2\highlight{\mc S_e}\sqrt{AK\ln(\highlight{|\mc S_e|}|\Acal| H^2K^2)}),
\end{equation}
holds $\forall s\in \mc S_e$, which completes the proof.
\end{proof}







==> texs/overview.tex <==
\section{Overview}
\label{sec:preliminary}
%\subsection{General Settings}
\vspace{-1em}
We consider an episodic Markov Decision process $\Mcal = (\Scal, \Acal, \Pstar, r, H)$ where $\Scal$ corresponds to the state space, $\Acal$ is the action space, $\Pstar$ is the transition operator, $r : \mathcal{S} \times \mathcal{A} \rightarrow[0,1]$ is the reward function and $H$ is the problem horizon. We use $|\Scal|,|\Acal|$ to denote the number of state and actions, and we use $\Pstar(\cdot|s,a)$ to denote the transition probability of state action pair $(s,a)$. The value function $V^\pi(s_0)$ of a policy $\pi$ starting at an initial state $s_0$ is defined as $V^\pi(s_0) := \bb E_\pi \brac{\sum_{h=0}^Hr(s_h,a_h)}$, where $\bb E_\pi$ denote the transition dynamic of $\Mcal$ under $\pi$. Similarly, $\Vstar(s_0)$ is the value function of the optimal policy $\pi^\star$. We consider a sequential interaction between a learner and the MDP $\mathcal{M}$ occurring in rounds indexed by $t \in \mathbb{N}$. At the start of round $t$ the learner selects a policy $\pi_t$ that is used to gather a sample trajectory from $\mathcal{M}$. As is standard in the literature, we measure the learner's performance up to round $T$ by ${\mathrm{Regret}(T) := \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)}$. 


\begin{wrapfigure}{r}{0.6\linewidth}
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
         \centering
            \includegraphics[width=1\textwidth]{Figures/Introduction/shaping-illu-maze.png}\vspace{-0.5em}
     \end{subfigure}
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
            \includegraphics[width=1\textwidth]{Figures/Introduction/shaping-illu-ucbvi.png}\vspace{-0.5em}
     \end{subfigure}
      \begin{subfigure}[t]{0.3\textwidth}
         \centering
            \includegraphics[width=1\textwidth]{Figures/Introduction/shaping-illu-ours.png}\vspace{-0.5em}
     \end{subfigure}
    \caption{\footnotesize{Reward shaping can allow for reduction of the ``effective'' state space size. In the above maze environment, the initial state is in the middle of the maze so finding the goal only requires solving half of the maze \textbf{(Left)}. While uninformed state covering exploration \textbf{(Middle)} would go both directions since it has no knowledge of goal location, effective shaping \textbf{(Right)} would allow for halving of the effective state space. The green circle represents the starting point and the red square represents the goal. Different colors represents the landscape of the shaped value function (green indicates smaller value and red indicates larger value).}}
    \label{fig:shaping-illustration}
    \vspace{-0.5em}
\end{wrapfigure}

Our objective is to show that knowing a reward shaping term $\Vtilde$ allows for significantly more sample efficient learning with high probability. More specifically, we show a sublinear regret upper bound with a leading term that depends on an ``effective state space'' of $\mathcal{M}$ which is determined by the quality of a reward shaping term $\Vtilde$ and the nature of the particular MDP being solved. This pruned effective state space can be much smaller than $|\Scal|$. Additionally, we will show an improved horizon dependence as the shaping term $\Vtilde$ allows for the bonus terms to be smaller and therefore decay faster thus replacing horizon factors of $H$ with $\beta \Vtilde$ ones. 

%%SL.5.18: Could expand on this (if true) to something like: 
%%SZ.5.19: Thanks for the suggestion, the new added part looks good!
% Our aim will be to show that, when the reward shaping function $\Vtilde$ satisfies our assumptions, the regret is sublinear for all $T \in \mathbb{N}$ and, more importantly, the leading term in the regret upper bound depends only on a notion of ``effective state space'' as measure by the quality of $\Vtilde$, rather than the entire state space $\Scal$.

% This is a significant departure from the conventional analysis on the efficiency of (uninformed) exploration methods, which typically only aims to show that the complexity is polynomial in the size of the state space $\Scal$. This is because without any additional information it is in general not possible to solve an RL task without visiting every state at least once, whereas appropriate reward shaping can provide precisely this kind of additional information.

Intuitively, reward shaping allows for the consideration of a reduced effective state space, consider the maze environment in Fig.~\ref{fig:shaping-illustration} with an agent starting in the middle. Without knowing where the goal is, an uninformed exploration algorithm needs to explore nearly the entire maze. However, an effectively incorporated reward shaping term $\Vtilde$ would allow an algorithm to prune out the entire left half of the grid, effectively halving the effective state space size. This can happen in two ways \textemdash firstly if the shaping can directly indicate that certain actions are sub-optimal then entire regions of the space can be eliminated from search. Secondly, even when the sub-optimal states are not eliminated, if their corresponding bonuses are scaled according to their shaped value $\Vtilde$ from the shaping rather than uniformly with $H$, it limits unnecessary exploration towards suboptimal states. 

% The bonus terms of an algorithm with $\beta\Vtilde$ scaling instead of $H$ will decay faster, thus if presented with the maze above it will explore suboptimal actions leading it to the left side of the board less often.

% The question becomes \textemdash what is an appropriate choice of $\Vtilde$ and how should it be incorporated into an RL algorithm would allow us to perform this type of effective state space reduction. 

%{\color{red}[TODO: Aldo we need to provide the H intuition, it's not in there now. IMPORTANT!!!!!!]}

% The intuition we want to capture in this work is that a $\Vtilde$ that contains accurate information about $\Vstar$ can help the learner detect the suboptimality of states and actions without the need to try these too many times and even without visiting them at all (e.g., without visiting states on the left when solving maze in Fig.\ref{fig:shaping-illustration} (a)). This allows the bulk of the learning to be focused on states and actions where $\Vtilde$ is not informative enough, or those lying within the support of the optimal policy. Thus, good approximate reward shaping terms $\Vtilde$ should enable the learner to prune sections of the state space and avoid wasting samples on clearly suboptimal states.

%%SL.5.18: Generally, I think the "effective state space" intuition above is great, but is this the only benefit? I thought we also had a more favorable horizon dependence? Perhaps we can add some discussion (maybe prior to the paragraph above?) that summarizes the different parts as something like this (if indeed this is true, but I might be misremembering since we iterated through several different bounds...):
% We will show that properly using a shaping term $\Vtilde$ provides multiple provably benefits in terms of the upper bound on sample complexity. First, it allows us to reduce the effective ``horizon'' of the problem, which otherwise shows up as a term in the bound. The intuition is that effective shaping reduces how much lookahead is needed to find a more optimal policy. Second, it allows us to derive a bound that is independent of the size of the state space, and instead depends on a notion of ``effective'' state space that removes any parts that are rendered clearly suboptimal by the shaping term, since these parts do not even need to be explored. Lastly, it [does something]

Based on this intuition, we propose slight modifications to a standard reinforcement algorithm that allows us to perform this analysis effectively. To aid our analysis, we introduce UCBVI-Shaped, a modification of the UCBVI algorithm~\citep{azar2017minimax} that uses an additional reward shaping term $\Vtilde$ in two ways: (1) Bonus scaling: $\Vtilde$ is used to provide an exploration bonus that combines inverse state visitation counts with reward shaping. This allows for the reduction of overoptimism and the dropping of the horizon $H$ dependence (2) Value projection: the shaping term is used to clip the empirical value function $\widehat{V}_h(s)$, which enables pruning unnecessary elements of the state space and allows for a bound that depends only on the effective state space size. 
% Appropriate use of the shaping information recovers the generic regret upper bounds achieved by UCBVI in Chapter 7 of~\cite{agarwal2019reinforcement}, and can improve upon them in case $\Vtilde$ contains meaningful information about $\Vstar$. We next provide a detailed description of UCBVI-Shaped and the resulting analysis in Section~\ref{sec:method} and ~\ref{sec:analysis}. 
Informally, our main result for UCBVI-Shaped can be summarized as follows:
\begin{theorem}[Informal Main Results] \label{theorem::informal_main}
With probability at least $1-\delta$, the regret of UCBVI - Shaped satisfies\footnote{Our main result, Theorem~\ref{theorem::main_result}, is slightly more complex than this statement. We have chosen this simplified form to aid the reader to form the right intuition. }
\begin{equation*}
\mathrm{Regret}(T)= \Ocal\left(  B(\Vtilde, \mathcal{M})\log(T/\delta) +\mathrm{Regret-UCBVI}(\Scal_{\mathrm{remain}}, \Acal, T)  \right) .
\end{equation*}
Here, $\Scal_{\mathrm{remain}}$ corresponds to the set of states in $\mathcal{M}$ where the information contained in $\Vtilde$ was not enough to rule them out, and $\mathrm{Regret-UCBVI}(\Scal_{\mathrm{remain}} \Acal, T)$ is a UCBVI regret upper bound function evaluated on $\Scal_{\mathrm{remain}}$ and $\Acal$. $B(\Vtilde, \mathcal{M})$ is a time-agnostic complexity measure that depends solely on the $\mathcal{M}$ and the quality of the shaping $\Vtilde$. 
\end{theorem}
%%SZ.5.19: the "-" in Regret-UCBVI is a bit confusing
%%SL.5.18: This is a reasonable start, but I have a few questions here: (1) "depends on solely on the MDP" is not super informative, because everything in the bound depends on the MDP -- is there something more precise we could say here? (2) is the second term literally just Regret-UCBVI? I thought it was a bit better than that?

We will define $\Scal_{\mathrm{remain}}$ and $B(\Vtilde, \mathcal{M})$ and describe their relationship to $\Vtilde$ precisely in Section~\ref{sec:analysis}. If $|\Scal_{\mathrm{remain}}| \ll |\Scal|$, the regret of UCBVI - Shaped can be substantially smaller than $\mathrm{Regret-UCBVI}(\Scal, \Acal)$, particularly since the first term of the regret grows logarithmically while the second scales with $\sqrt{T}$. We state our assumptions next:
%\vspace{-0.5em}

% \paragraph{Assumptions.} The quality of the shaping term $\Vtilde$ is described by a parameter $\beta$:

\begin{assumption}\label{assump::sandwich}
The quality of the shaping term $\Vtilde$ is described by a parameter $\beta$. We assume access to shaping ``value function'' estimators $\widetilde{V}_h: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ such that, $\Vtilde_h(s)  \leq \Vstar_h(s)  \leq \beta \Vtilde_h(s)$, for all $s \in \Scal$, $h \in [H]$ and for some $ \beta \geq 1$.
\end{assumption}

% For simplicity we will also assume the rewards are deterministic and have support in $[0,1]$. 
% This assumption does not limit the analysis and can be easily removed at a cost of a $\Ocal(\sqrt{T})$ in our regret bounds. 

\begin{assumption}\label{assump::rewards}
We assume the reward functions satisfy ${r(s,a) \in [0,1]},\forall (s, a) \in \Scal\times \Acal.$
\end{assumption}

\begin{assumption}\label{assump::h_indexing}
The states $\Scal$ are $h-$indexed, i.e., the states reachable at time $h \in [H]$ are disjoint from the states reachable at time $h' \in [H]$ when $h \neq h'$. 
\end{assumption}\vspace{-0.5em}




% The primary observation we are aiming to capture in our results is that having knowledge of an approximation $\Vtilde$ satisfying Assumption~\ref{assump::sandwich}
% should enable the learner \aldo{I use this `learner' language} to prune sections of the state space and avoid spending many samples learning the MDP dynamics in suboptimal states.
% In this case the cost of learning, which we quantify via regret, should then scale with the size of the effective dimension of the state space, and not with the size of $\Scal$. Our objective is to provide a simple characterization of this depending only on the quality of $\Vtilde$ and the MDP $\mathcal{M}$ and an algorithm satisfying a regret guarantee whose state dependence scales with this quantity. 


\paragraph{Contributions.} Our analysis introduces the notions of pseudosuboptimal and path-pseudosuboptimal states to quantify the ``effective'' size of the state space as a function of the quality of the shaping term $\Vtilde$, and we use these notions to show how UCBVI-Shaped can attain significantly improved regret rates. We further show that incorporating shaping into the exploration bonus term improves the horizon-dependence in the bound when the shaping is good enough, allowing us to replace a leading $H$ term with $\max_s \beta \Vtilde(s)$. 

% We confirm these findings with numerical simulations on tabular MDPs.

==> texs/proofs.tex <==
\newpage
\section{Full Proofs}
\label{sec:supporting_lemmas}


% \subsection{Old stuff from main}




% We start by showing that we can bound $N_h^t(s,a)$ for all $t$, and for all $(s,a) \in \pathpseudosub_\Delta \times \mathcal{A}$ for all $\Delta > 0$. For that let's consider the value iteration formula at time $t$ for an arbitrary state action pair $(s,a)$ , 
% \begin{equation*}
%     \Qhat_h^t(s,a)  =  r(s,a) + b_h^t(s,a) + \Phat_t(\cdot |s,a) \cdot \Vhat_{h+1}^t \leq r(s,a) +   b_h^t(s,a) + \beta \Phat_t(\cdot |s,a) \cdot \Vtilde_{h+1}
% \end{equation*}


% The last corollary implies that once $b_h^t(s,a) + \tilde{b}_h^t(s,a) <  \Vstar(s) - \Qtilde^u(s,a)$ optimism guarantees that from that point on, action $a$ will never again be taken at state $s$.
% \aldo{Write some intution about what this implies and how it implies the following result}






% The proof of Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub} can be found in Appendix~\ref{appendix::proof_lemma_upper_bound_visitation}. 


% Now we are ready to use these results in proving our regret bounds. Equation~\eqref{equation::neighbors_restricted} implies that,

% \begin{lemma}\label{lemma::path_pseudo_upper_bound_phat_pstar}
% Fix $\delta\in (0,1)$, $\forall t\in [1,2,\dots T]$, $(s, a) \in \Scal \backslash ( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$, $h\in [0,1,\dots,H-1]$, with probability at least $1-\delta$:

% \begin{align*}
%     \abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}} &\leq 16 \beta \cdot \sqrt{ \frac{ |\Scal \backslash \pathpseudosub_\Delta |  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\Vtilde^2_{h+1}(s') | s,a]  \ln\frac{ 8 \Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_t(s,a) }} +\\
%     &\quad  \frac{12\beta \Vtildemax_{h+1} }{N_t(s,a)}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|t^3}{\delta}.
% \end{align*}
% For all $\{f_h: \Scal \rightarrow \mathbb{R}\}_{h = 0}^{H-1}$ such that $f_h(s) \in \left[ \Vtilde_h, \beta \Vtilde_h\right]$ simultaneously and where $\widehat{\mathrm{Var}}(f_{h+1}(s') | s,a)  = \frac{1}{N_h^k(s,a)( N_h^k(s,a)-1)} \sum_{1 \leq i < j < N_h^k(s,a)} (f_{h+1}(s_{h+1}^i) - f_{h+1}(s_{h+1}^j))^2$. 

% %\aldo{All those $\log |\Scal|$ terms may be able to be reduced to $\log |\Scal \backslash \pathpseudosub_\Delta | $.}

% \end{lemma}



% \begin{proof}
% This is a simple consequence of Equation~\eqref{equation::neighbors_restricted}. For all state action pairs $(s, a) \in \Scal \backslash ( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$, we have that $\neighbor(s,a) \subseteq \Scal \backslash \pathpseudosub_\Delta$. Therefore, the support of $\Pstar(\cdot | s,a )$ and $\Phat_t(\cdot | s,a) $ is contained in $\Scal \backslash \pathpseudosub_\Delta$. Thus, despite the functions $f$ being defined for all $\Scal$, for the purpose of the lemma, only their values over states in $\Scal \backslash \pathpseudosub_\Delta$ matter. This result is an immediate consequence of Lemma~\ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} but instead using a union bound over $\{f_h: \Scal \backslash \pathpseudosub_\Delta \rightarrow \mathbb{R}\}_{h = 0}^{H-1}$.   
% \end{proof}



% The results of Lemmas~\ref{lemma::path_pseudo_upper_bound_phat_pstar} and~\ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} can be used to upper bound 



% \aldo{finalize the description of the proof of Theorem~\ref{theorem::main_result}. Comment why we needed to modify UCBVI and not something like UCRL. MEntion why UCBVI along is not enough even if it is amicable to sparse transition probability matrices}



% \subsection{All stuff}








Let $f_h : \Scal \rightarrow \mathbb{R}$ be an arbitrary family of horizon indexed functions satisfying $\| f_h \|_\infty \leq B$ for some $B > 0$. For the following lemma we assume $f_h$ is not a random variable but simply a fixed function of $\Scal$ . The following upper bounds hold,

\begin{lemma}\label{lemma::fixed_f_bound}
Fix $\delta \in (0,1)$, $\forall t \in \mathbb{N}$, $s \in \Scal$, $a \in \Acal$ and $h \in [0, \cdots, H-1]$, with probability at least $1-\delta$,
\begin{align*}
       \abs{\Phat_h^t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}} 
      &\leq 16 \sqrt{ \frac{ \mathrm{Var}(f_{h+1}(s') | s,a) \ln \frac{2|\Scal||\Acal|t}{\delta} }{ N_h^t(s,a)} } + \frac{12B\frac{2|\Scal||\Acal|t}{\delta}}{N_h^t(s,a) } \\
      &\leq 16B \sqrt{ \frac{ \ln \frac{2|\Scal||\Acal|t}{\delta} }{ N_h^t(s,a)} } + \frac{12B\frac{2|\Scal||\Acal|t}{\delta}}{N_h^t(s,a) } 
\end{align*}
% \aldo{add an $H$ to the logarithm in the square root.}
 for all $t \in \mathbb{N}$. Similarly with probability at least $1-\delta$,
\begin{equation*}
       \abs{\Phat_h^t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}} \leq 16 \sqrt{ \frac{ \widehat{\mathrm{Var}}(f_{h+1}(s') | s,a) \ln \frac{2|\Scal||\Acal|t}{\delta} }{ N_h^t(s,a)} } + \frac{12B\frac{2|\Scal||\Acal|t}{\delta}}{N_h^t(s,a) }
\end{equation*}
 for all $t \in \mathbb{N}$. Where $\widehat{\mathrm{Var}}(f_{h+1}(s') | s,a)  = \frac{1}{N_h^k(s,a)( N_h^k(s,a)-1)} \sum_{1 \leq i < j < N_h^k(s,a)} (f_{h+1}(s_{h+1}^i) - f_{h+1}(s_{h+1}^j))^2$.
\end{lemma}


\begin{proof}
Consider a fixed tuple $s,a,t, h \in \Scal \times \Acal \times \mathbb{N} \times [0, \cdots, H-1]$. By the definition of $\Phat_h^t$ we have,
\begin{equation*}
     \Phat_h^t(\cdot|s,a)^\top f_{h+1} = \frac{1}{N_h^t(s,a)}\sum_{i=1}^{t-1} 
     \indicator{(s_{h'}^i,a_{h'}^i) = (s,a)}f_{h+1}(s_{h'+1}^i).
\end{equation*}


Now denote $\mathcal{H}_{h,i}$ as the entire history from $t=0$ to iteration $t=i$ where in iteration $i$, the history $\mathcal{H}_{h,i}$ includes all interactions from step $0$ up to and including time step $h$. Next, $\forall i = 0,1,\dots,t-1$, define the random variables, 

\begin{equation*}
    X_{i, h'}(s,a) = \indicator{(s^i_{h'},a^i_{h'})=(s,a)}f_{h+1}(s^i_{h'+1}) - \bb E\brac{\indicator{(s^i_{h'},a^i_{h'})=(s,a)}f_{h+1}(s^i_{h'+1})|\mc H_{h,i}}.
\end{equation*}


Notice that $\abs{X_{i, h'}}\leq B$, if $\indicator{(s_{h'}^i,a_{h'}^i)=(s,a)}=1$, else $\abs{X_{i,h'}} = 0$ so that 

\begin{equation*}
    \mathrm{Var}(  X_{t, h}(s,a)  | H_{h-1,t}) \leq \begin{cases}
    0 &\text{if } \abs{X_{i,h'}} = 0 \\
    B^2 &\text{o.w.}
    \end{cases}
\end{equation*}

An anytime Bernstein bound (see Lemma~\ref{lemma:simplified_freedman}) implies,

\begin{align*}
  \abs{\sum_{i=1}^{t-1} 
      X_{i, h'}(s,a) } &\leq 16 \sqrt{ N_h^t(s,a) \mathrm{Var}( f_{h+1}(s')  | s,a)  \ln \frac{2|\Scal||\Acal|t}{\delta}  } + 12B\frac{2|\Scal||\Acal|t}{\delta} \\
      &\leq 16 B\sqrt{ N_h^t(s,a) \ln \frac{2|\Scal||\Acal|t}{\delta}  } + 12B\frac{2|\Scal||\Acal|t}{\delta}.
\end{align*}
With probability at least $1-\delta$ for all $t \in \mathbb{N}$. Thus, 

\begin{equation*}
   \abs{\Phat_h^t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}} \leq 16B \sqrt{ \frac{ \ln \frac{2|\Scal||\Acal|t}{\delta} }{ N_h^t(s,a)} } + \frac{12B\frac{2|\Scal||\Acal|t}{\delta}}{N_h^t(s,a) }
\end{equation*}
With probability at least $1-\delta$ for all $t \in \mathbb{N}$. The second inequality can be proven following the exact same proof process as described above, but instead making use of the empirical Bernstein bound of~\ref{lemma::bernstein_anytime} instead. 












\end{proof}


The following bound relates the error of $\Phat_t$ and $\Pstar$. 

\begin{corollary}[State-action wise model error under $\Vstar$ (Lemma 7.3 of~\cite{agarwal2019reinforcement})]
\label{corollary:ModelErrorEmpiricalBernsteinV}
Fix $\delta\in (0,1)$, $\forall t\in [1,2,\dots T],s\in \Scal,a\in \Acal,h\in [0,1,\dots,H-1]$, consider $\forall \Vstar_h:\Scal \rightarrow [0,H]$ with probability at least $1-\delta$:

\begin{equation*}
    \abs{\Phat_t(\cdot|s,a)^\top \Vstar_{h+1} - \Pstar(\cdot|s,a)^\top \Vstar_{h+1}} \leq 16\sqrt{ \frac{ \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a)  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta} }{ N_h^t(s,a) }} + \frac{12\Vstarmax }{N_h^t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta}.
\end{equation*}
for all $t \in \mathbb{N}$. Where $\widehat{\mathrm{Var}}(\Vstar_{h+1}(s') | s,a)  = \frac{1}{N_h^k(s,a)( N_h^k(s,a)-1)} \sum_{1 \leq i < j < N_h^k(s,a)} (\Vstar_{h+1}(s_{h+1}^i) - \Vstar_{h+1}(s_{h+1}^j))^2$ and $\Vstarmax = \max_{s } \Vstar(s)$. 

\aldo{Do we want to use $H$ in this bonus? It doesn't look like $b_h^t(s,a)$ is defined with $H$}

\end{corollary}



\begin{proof}
A direct application of Corollary~\ref{lemma::fixed_f_bound} using $B = \Vstarmax$ yields the desired result. 
\end{proof}





A direct consequence of Lemma~\ref{corollary:ModelErrorEmpiricalBernsteinV} and Assumption~\ref{assump::sandwich} is that, 

\begin{corollary}\label{corollary::variance_bonus_domination}
The $\Vstar$ ``variance bonus'' is upper bounded by the empirical $\Vtilde$ ``second moment bonus''.

\begin{equation*}
    16\sqrt{ \frac{ \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a)  \ln\frac{ 2 |\Scal||\Acal|t}{\delta} }{ N_t(s,a) }}  \leq 16 \beta \cdot \sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\Vtilde^2_{h+1}(s') | s,a ]  \ln\frac{ 2 |\Scal||\Acal|}{\delta} }{ N_t(s,a) }} 
\end{equation*}
and 

\begin{equation*}
    \frac{12\Vstarmax }{N_h^t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta} \leq \frac{12\beta \Vtildemax }{N_h^t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta}
\end{equation*}
\end{corollary}

\begin{proof}
For any random variable $X \sim \mathbb{P}$, 
\begin{equation*}
    \mathrm{Var}(X) \leq \mathbb{E}_{X \sim \mathbb{P}}\left[ X^2 \right]. 
\end{equation*}
Therefore, for all $s,a$ and any empirical distribution $\Phat_t(\cdot | s,a)$,

\begin{equation*}
    \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a) \leq \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }\left[\left(\Vstar_{h+1}(s') \right)^2| s,a\right]
\end{equation*}

Finally, by Assumption~\ref{assump::sandwich},

\begin{equation*}
    \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }\left[\left(\Vstar_{h+1}(s') \right)^2| s,a\right] \leq \beta^2 \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }\left[\Vtilde^2_{h+1}(s')| s,a\right].
\end{equation*}
The result follows.
\end{proof}





Define as $\Vhat_{h}^t$ to the stage $h$ value function of $\pi_t$ as computed in the learned model and using bonus augmented rewards (with bonuses defined as in~\ref{eq::shaped_bonus}) with the data collected up to round $t-1$. We start by showing that $\Vhat_h^t$ is always larger than $\Vstar_h(s)$


We show the following supporting Lemma, a generalization of Lemma~\ref{lemma::fixed_f_bound}.   





\begin{lemma}
\label{lemma:ModelErrorEmpiricalBernsteinGeneralized}
Fix $\delta\in (0,1)$, $\forall t\in [1,2,\dots, T],s\in \Scal,a\in \Acal,h\in [0,1,\dots,H-1]$,  with probability at least $1-\delta$:

\begin{align*}
      &\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}}\\
      \leq &\;16 \beta \cdot \sqrt{ \frac{| \mathrm{support}( \Pstar(\cdot |s,a) )| \widehat{\bb E}_{s' \sim \Phat_t(\cdot | s,a) }[\tilde{V}^2_{h+1}(s') | s,a]  \ln\frac{ 8B |\Scal| |\Acal| t^3}{\delta} }{ N_t(s,a) }} \\
      &+\quad\frac{12B| \mathrm{support}( \Pstar(\cdot |s,a) )|}{N_t(s,a)}\ln \frac{ 8B |\Scal| |\Acal|t^3}{ \delta} + \frac{1}{t^2}
\end{align*}
Simultaneously for all $\{f_h: \Scal \rightarrow \mathbb{R}\}_{h = 0}^{H-1}$ such that $f_h(s) \in \left[ \Vtilde_h, \beta \Vtilde_h\right]$ and $\| f_h\|_\infty \leq B$. Where $\mathrm{support}( \Pstar(\cdot |s,a) ) $ corresponds to the size of the support of distribution $\Pstar(\cdot |s,a)$. %and where $\widehat{\mathrm{Var}}(f_{h+1}(s') | s,a)  = \frac{1}{N_h^k(s,a)( N_h^k(s,a)-1)} \sum_{1 \leq i < j < N_h^k(s,a)} (f_{h+1}(s_{h+1}^i) - f_{h+1}(s_{h+1}^j))^2$. 

\end{lemma}





\begin{proof}


The same proof template as in Lemma~\ref{lemma::fixed_f_bound} plus a union bound over a covering of the space of $f$ functions yields the desired result. Note that for all $s, a \in \Scal \times \Acal$,
\begin{equation*}
    \widehat{\mathrm{Var}}(f_{h+1}(s') | s,a) \leq \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[f^2_{h+1}(s') | s,a] \leq \beta^2 \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\Vtilde^2_{h+1}(s') | s,a]
\end{equation*}

Therefore Lemma~\ref{lemma::fixed_f_bound} implies that for any fixed $f_{h+1}$, with probability at least $1-\delta'$

\begin{align}
    \label{eq::single-point-convergence}    
        &\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}}\\
        \leq&\; 16 \beta \cdot \sqrt{ \frac{ \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(f_{h+1}(s') | s,a)  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta'} }{ N_t(s,a) }} + \frac{12B}{N_t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta'} \notag\\
        \leq &\;16 \beta \cdot \sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\tilde{V}^2_{h+1}(s') | s,a]  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta'} }{ N_t(s,a) }} +  \frac{12B}{N_t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta'} 
\end{align}



for all (fixed) $f \in \{f_h: \Scal \rightarrow \mathbb{R}\}_{h = 0}^{H-1}$ and for all $s, a, h \in \Scal \times \Acal \times H$ simultaneously.  We now apply a standard $\epsilon-$net covering argument to the inequality we have proven above. Notice that regardless of the number of samples, $\mathrm{support}( \Phat_t(\cdot |s,a) ) \subseteq \mathrm{support}( \Pstar(\cdot |s,a) )$. Thus, the only ``entries'' that matter in $f_{h+1}$ are those corresponding to states in $\mathrm{support}( \Pstar(\cdot |s,a) )$. 

Let's consider an $\epsilon-$net of $f_{h+1}$ restricted to $\mathrm{support}( \Pstar(\cdot |s,a) )$. Since for any $s \in\Scal$, we assume $f_{h+1} \in [\Vtilde_{h+1}, \beta \Vtilde_{h+1}]$, there exists an epsilon net $\mathcal{N}_\epsilon$ under the infinity norm satisfying $|\mathcal{N}_\epsilon| \leq (\frac{2B}{\epsilon})^{| \mathrm{support}( \Pstar(\cdot |s,a) )|}$. For any $f_{h+1}$ we denote by $f_{h+1}^\epsilon$ its closest element in $\mathcal{N}_\epsilon$ (in the infinity norm over $\mathrm{support}( \Pstar(\cdot |s,a) )$). The following holds, 

\begin{align*}
     \left|\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}}  -  \abs{\Phat_t(\cdot|s,a)^\top f^\epsilon_{h+1} - \Pstar(\cdot|s,a)^\top f^\epsilon_{h+1}} \right| \leq  \\
     \abs{\Phat_t(\cdot|s,a)^\top f_{h+1}- \Phat_t(\cdot|s,a)^\top f_{h+1}} + \abs{\Pstar(\cdot|s,a)^\top f^\epsilon_{h+1} - \Pstar(\cdot|s,a)^\top f^\epsilon_{h+1}} \leq      2\epsilon.
\end{align*}

And therefore, setting $\delta' = \frac{\delta}{(\frac{2B}{\epsilon})^{| \mathrm{support}( \Pstar(\cdot |s,a) )|}} \leq \frac{\delta}{|\mathcal{N}_\epsilon|} $, a union bound over all elements of $\mathcal{N}_\epsilon$ implies that with probability at least $1-\delta$,

\begin{align*}
      &\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}}\\
      \leq &\;16 \beta \cdot \sqrt{ \frac{| \mathrm{support}( \Pstar(\cdot |s,a) )| \widehat{\bb E}_{s' \sim \Phat_t(\cdot | s,a) }[\tilde{V}^2_{h+1}(s') | s,a]  \ln\frac{ 4B |\Scal| |\Acal| t}{\epsilon\delta} }{ N_t(s,a) }}\\
      &+\frac{12B| \mathrm{support}( \Pstar(\cdot |s,a) )|}{N_t(s,a)}\ln \frac{ 4B |\Scal| |\Acal|t}{\epsilon\delta} + 2\epsilon
\end{align*}


for all $f_{h+1}$ simultaneously. Setting $\epsilon = \frac{1}{2t^2}$ we get that with probability at least $1-\delta$,



\begin{align*}
      &\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}}\\
      \leq &\; 16 \beta \cdot \sqrt{ \frac{| \mathrm{support}( \Pstar(\cdot |s,a) )| \widehat{\bb E}_{s' \sim \Phat_t(\cdot | s,a) }[\tilde{V}^2_{h+1}(s') | s,a]  \ln\frac{ 8B |\Scal| |\Acal| t^3}{\delta} }{ N_t(s,a) }} \\
      &+\frac{12B| \mathrm{support}( \Pstar(\cdot |s,a) )|}{N_t(s,a)}\ln \frac{ 8B |\Scal| |\Acal|t^3}{ \delta} + \frac{1}{t^2}
\end{align*}

for all $f_{h+1}$ simultaneously and for all $t \in \mathbb{N}$. This completes the result.












% To conclude we apply the same reasoning that gave us Corollary~\ref{corollary::variance_bonus_domination}. 

% \simon{I have added the $\eps$-net covering for all $f$, assuming double $\ln$ in \eqref{eq::single-point-convergence} is correct (although I am not too sure about it, I guess it should be $2|\Scal||\Acal|t/\delta$ instead of $\ln( 2|\Scal||\Acal|t/\delta)$).}
% {\bf $\eps$-net covering for all $f$.} Note that $\norm{f}{2}\leq \beta H\sqrt{|\Scal|}$ for any $f:\mc S\mapsto\left[ \Vtilde_h, \beta \Vtilde_h\right]$. A standard $\eps$-net argument shows that we can \highlight{construct an $\eps$-net $\mc N_\eps$ over $\left[ \Vtilde_h, \beta \Vtilde_h\right]^{|\Scal|}$ with $\abs{\mc N_\eps}\leq(1+2\beta H\sqrt{|\Scal|}/\eps)^{|\Scal|}$}, such that for any $f\in \left[ \Vtilde_h, \beta \Vtilde_h\right]^{|\Scal|}$, there exists a point $f^\prime\in \mc N_\eps$, such that $\norm{f-f^\prime}{2}\leq \eps$. Note that the $\eps$-net $\mc N_\eps$ is independent of the training data during the learning process. Now applying \eqref{eq::single-point-convergence} and a union bound over all $f$ in $\mc N_\eps$, we have that with probability at least $1-\delta$, for all $s,a,t$ and $\forall f\in \mc N_\eps$, we have
% \begin{equation}
%     \begin{split}
%         &\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}} \\
%         \leq &16 \sqrt{\left( \frac{3\beta^2}{2} - \frac{1}{2}\right) } \cdot \sqrt{ \frac{\highlight{|\Scal|} \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\tilde{V}_{h+1}(s') | s,a)  \ln\paren{\frac{ 2 |\Scal| |\Acal| t}{\delta}\highlight{(1+\beta H\sqrt{|\Scal|}/\eps)}} }{ N_t(s,a) }}\\
%         &+ \quad \frac{12H\highlight{|\Scal|}}{N_t(s,a)}\ln \paren{\frac{ 2 |\Scal| |\Acal|t}{\delta}\highlight{(1+2\beta H\sqrt{|\Scal|}/\eps)}}
%     \end{split}
% \end{equation}
% Finally, for all $f\in [0,H]^S$, denote its closest point in $\mc N_\eps$ as $f^\prime$, we have 

% \begin{equation*}
%     \begin{split}
%         &\abs{\Phat_t(\cdot|s,a)^\top f_{h+1} - \Pstar(\cdot|s,a)^\top f_{h+1}}\\
%         \leq & \abs{\frac{\sum_{i=0}^{t-1}\indicator{(s_h^i,a_h^i)=(s,a)}f^\prime(s_{h+1}^i)}{N_h^t(s,a)} - \bb E_{s^\prime \sim P_h^\star(s,a)}f^\prime(s^\prime) } + \abs{\bb E_{s^\prime \sim P_h^\star(s,a)}(f(s^\prime )-f^\prime(s^\prime))}\\
%         &+ \abs{\frac{\sum_{i=0}^{t-1}\indicator{(s_h^i,a_h^i)=(s,a)}(f(s_{h+1}^i)- f^\prime(s^i_{h+1}))}{N_h^t(s,a)} }\\
%         \leq &32 \sqrt{\left( \frac{3\beta^2}{2} - \frac{1}{2}\right) } \cdot \sqrt{ \frac{\highlight{|\Scal|} \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\tilde{V}_{h+1}(s') | s,a)  \ln\paren{\frac{ 2 |\Scal| |\Acal| t}{\delta}\highlight{(1+\beta H\sqrt{|\Scal|}/\eps)}} }{ N_t(s,a) }}\\
%         &+ \quad \frac{24H\highlight{|\Scal|}}{N_t(s,a)}\ln \paren{\frac{ 2 |\Scal| |\Acal|t}{\delta}\highlight{(1+2\beta H\sqrt{|\Scal|}/\eps)}} + 2 \eps
%     \end{split}
% \end{equation*}
% where the last inequality hold because $\norm{f-f^\prime}{2}\leq \eps$, hence $\abs{f(s) - f^\prime(s)}\leq \eps,\forall s\in \mc S$. Now if we set $\eps = 1/T$ and use the fact that $N_h^t(s,a)\leq T$, we have
% \begin{equation}
%     \begin{split}
%         &\abs{\frac{\sum_{i=0}^{k-1}\indicator{(s_h^i,a_h^i)=(s,a)}f(s_{h+1}^i)}{N_h^t(s,a)} - \bb E_{s^\prime \sim P_h^\star(s,a)}f(s^\prime) }\\
%         \leq &32 \sqrt{\left( \frac{3\beta^2}{2} - \frac{1}{2}\right) } \cdot \sqrt{ \frac{\highlight{|\Scal|} \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\tilde{V}_{h+1}(s') | s,a)  \ln\paren{\frac{ |\Scal| |\Acal| t}{\delta}\highlight{(1+\beta H\sqrt{|\Scal|}/\eps)}} }{ N_t(s,a) }}\\
%         &+ \quad \frac{24H\highlight{|\Scal|}}{N_t(s,a)}\ln \paren{\frac{ |\Scal| |\Acal|t}{\delta}\highlight{(1+2\beta H\sqrt{|\Scal|}/\eps)}} + \frac{2}{T}\\
%         \leq &32 \sqrt{\left( \frac{3\beta^2}{2} - \frac{1}{2}\right) } \cdot \sqrt{ \frac{\highlight{|\Scal|} \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\tilde{V}_{h+1}(s') | s,a)  \ln\paren{\frac{ 2 |\Scal| |\Acal| t}{\delta}\highlight{(1+\beta H\sqrt{|\Scal|}/\eps)}} }{ N_t(s,a) }}\\
%         &+ \quad \frac{\highlight{26}H\highlight{|\Scal|}}{N_t(s,a)}\ln \paren{\frac{ 2 |\Scal| |\Acal|t}{\delta}\highlight{(1+2\beta H\sqrt{|\Scal|}/\eps)}},
%     \end{split}
% \end{equation}
% which completes the proof.
\end{proof}




\subsection{Proof of Lemma~\ref{lemma::optimism}}\label{appendix::lemma_optimism_proof}


\begin{proof}
We prove via induction. At the additional time step $H$ we have $\Vhat_H^t(s) = \Vstar_H(s) = 0$ for all $s$. 

Starting at $h+1$, and assuming we have $\Vhat_{h+1}^t (s) \geq \Vstar_{h+1}(s)$ for all $s$, we move to $h$ below.

Consider any $s, a \in \Scal \times \Acal$. First if $\Qhat_h^t(s,a) = H$ then we have $\Qhat_h^t(s,a) \geq \Qstar_h(s,a)$. The following inequalities hold,


\begin{align*}
    \Qhat_h^t(s,a) - \Qstar_h(s,a) &= b_h^t(s,a) + \Phat_t(\cdot |s,a) \cdot \Vhat_{h+1}^t - \Pstar(\cdot | s,a) \cdot \Vstar_{h+1}\\
    &\stackrel{(i)}{\geq} b_h^t(s,a) + \Phat_t(\cdot |s,a) \cdot \Vstar_{h+1} - \Pstar(\cdot | s,a) \cdot \Vstar_{h+1}\\
    &=  b_h^t(s,a) + \left(\Phat_t(\cdot |s,a)  - \Pstar(\cdot | s,a) \right)\cdot \Vstar_{h+1} \\
    &\stackrel{(ii)}{\geq} b_h^t(s,a) - 16\sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\Vtilde^2_{h+1}(s') | s,a ]  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta} }{ N_t(s,a) }} - \frac{12\Vtildemax }{N_t(s,a)}\ln \frac{ 2 |\Scal||\Acal|t}{\delta} \\
    &\stackrel{(iii)}{\geq} 0
\end{align*}

Where $(i)$ holds because of the inductive optimism assumption. Inequality $(ii)$ holds because of Lemma~\ref{corollary:ModelErrorEmpiricalBernsteinV} and $(iii)$ because of corollary~\ref{corollary::variance_bonus_domination}. 




\end{proof}




The following Lemma will be useful in the coming sections,
\begin{lemma}\label{lemma::indicator_upper_bound_regret}
Let $\mathcal{U} \subseteq \Scal \times \Acal$ be an arbitrary subset of $\Scal \times \Acal$. With probability at least $1-\delta$,

\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  \leq \qquad \qquad \qquad \qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad \qquad  \qquad \qquad  \\
    \qquad \sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} -\Vstar_{h+1}\right)\right)+ \\
    \qquad  \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \qquad \qquad \qquad \qquad \qquad\qquad \qquad \quad
\end{align*}
And
\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  \leq  \qquad \qquad \qquad \qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad  \qquad \qquad \\
    \qquad \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) \right) + \\
    \qquad \sum_{t=1}^t\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \qquad \qquad \qquad \qquad \qquad\qquad \qquad 
\end{align*}
% \aldo{Some of the $H$ dependence here can probably be turned into a $\Vtildemax$}

% \textbf{Note:} An anytime bound is also possible. \aldo{consider changing this result to be anytime.}
\end{lemma}




\begin{proof}


First note that by the simulation lemma, optimism (see Equation~\ref{equation::simulation_optimism}) and by Hoeffding inequality. 

\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) &\leq \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \paren{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}}  \right]\\
    &\leq \sum_{t=1}^T \sum_{h=1}^H \paren{b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}}  + \Ocal\left(H\sqrt{ TH \ln(T/\delta)   }     \right)
\end{align*}
with probability at least $1-\delta$. The inequality above is satisfied because
\begin{align*}
\abs{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}  }\leq 2H     
\end{align*}

We will now 



\aldo{We now turn to bounding the trajectory based stuff}


% \aldo{this $H$ dependence can probably be traded with a $\max \Vtilde$ one}. 
Next notice that $\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t}   \leq 2H^2$ and therefore, 

\begin{align*}
    &\sum_{t=1}^T \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \\
    \leq&\;\sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)+  \sum_{t=1}^t \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  
\end{align*}

Similarly, 
\begin{align*}
    &\sum_{t=1}^T \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \\
    \leq&\;\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \sum_{t=1}^T\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H
\end{align*}

The result follows.
% Finally, let's prove an upper bound for $\Qstar(s,\pi_\star(s)) - \Qstar(s,\pi_t(s))$. 

% \begin{align*}
%     \Qstar_h(s,\pi_\star(s) ) - \Qstar_h(s,\pi_t(s)) &\stackrel{(i)}{\leq} \Qhat_h^t(s,\pi_t(s) ) - \Qstar_h(s,a) \\
%     &= \Phat_t(\cdot | s, \pi_t(s) )^\top \Vhat_{h+1}^t - \Phat_t(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} +   \Phat_t(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} - \Pstar(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} \\
%     &\leq \Phat_t(\cdot | s, \pi_t(s) )^\top \Vhat_{h+1}^t  - 
% \end{align*}
% Inequality $(i)$ holds because of optimism of $\Qhat_h^t(s,\pi_\star(s) )$. 





\end{proof}


\aldo{More refined version of this decomposition lemma. }


The following Lemma will be useful in the coming sections,
\begin{lemma}\label{lemma::indicator_upper_bound_regret_refined_version}
Let $\mathcal{U} \subseteq \Scal \times \Acal$ be an arbitrary subset of $\Scal \times \Acal$. With probability at least $1-\delta$,

\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) \right)+ \right.\\
    &\quad \left.\sum_{t=1}^t \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  \right] 
    + \Ocal\left( \mathbb{E}_{\tau \sim \pi_t} \left[\sum_{h=1}^H b_h^t(s_h,a_h)\right] \right)%\\
    %&\quad \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
\end{align*}
And
\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq 
    \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[   \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right)\right) + \right.\\
    &\quad \left.\sum_{t=1}^T\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H \right] + \Ocal\left( \mathbb{E}_{\tau \sim \pi_t} \left[\sum_{h=1}^H b_h^t(s_h,a_h)\right] \right)
    %\\
    % &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    % &\quad \sum_{t=1}^t\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
\end{align*}
% \aldo{Some of the $H$ dependence here can probably be turned into a $\Vtildemax$}

% \textbf{Note:} An anytime bound is also possible. \aldo{consider changing this result to be anytime.}
\end{lemma}




\begin{proof}






First note that by optimism  and the simulation lemma (see Equation~\ref{equation::simulation_optimism}). 

\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) &\leq \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \paren{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}}  \right]\\
    &= \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \paren{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} - \Vstar_{h+1} + \Vstar_{h+1} \right)}  \right] \\
    &=\sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \paren{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} - \Vstar_{h+1} \right)}  \right]  \\
    &\quad + \underbrace{\mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot  \Vstar_{h+1}  \right]  }_{\mathrm{I}}
    % &\leq \sum_{t=1}^T \sum_{h=1}^H \paren{b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}}  + \Ocal\left(H\sqrt{ TH \ln(T/\delta)   }     \right)
\end{align*}


Let's bound term $\mathrm{I}$ using Corollary~\ref{corollary:ModelErrorEmpiricalBernsteinV} . 
\begin{align*}
    \mathrm{I} &= \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right)^\top \cdot  \Vstar_{h+1}  \right]  \\
     & \stackrel{(i)}{=} \Ocal\left( \mathbb{E}_{\tau \sim \pi_t}\left[  \sum_{h=1}^H  \sqrt{ \frac{ \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s_h,a_h) }(\Vstar_{h+1}(s') | s_h,a_h)  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta} }{ N_h^t(s_h,a_h) }} + \frac{12H}{N_h^t(s_h,a_h)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta} \right] \right)\\
     &= \Ocal\left( \mathbb{E}_{\tau \sim \pi_t} \left[\sum_{h=1}^H b_h^t(s_h,a_h)\right] \right)
\end{align*}
with probability at least $1-\delta$ for all $t, s_h$ ad $a_h$ simultaneously. Inequality $(i)$ holds as a consequence of Corollary~\ref{corollary:ModelErrorEmpiricalBernsteinV}. \aldo{Check the use of this corollary. The low order term depends on $H$.}

Now observe that
\begin{align*}
\abs{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t}- \Vstar_{h+1}\right)  }&\leq 2H     \\
 \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) &\leq 2H^2
 \end{align*}
 \aldo{Change these to $\Ocal$ notation?}
 and therefore, 
\begin{align*}
    &\sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) \right] \\
    \leq&\;\sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} -\Vstar_{h+1}\right) \right)  +\right.\\
    &\quad \left.\sum_{t=1}^t \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  \right]
\end{align*}

Similarly, 
\begin{align*}
    &\sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[  \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) \right]\\
    \leq&\;\sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[   \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right)\right) +\right.\\
    &\left.\sum_{t=1}^T\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H \right]
\end{align*}

The result follows.
% Finally, let's prove an upper bound for $\Qstar(s,\pi_\star(s)) - \Qstar(s,\pi_t(s))$. 

% \begin{align*}
%     \Qstar_h(s,\pi_\star(s) ) - \Qstar_h(s,\pi_t(s)) &\stackrel{(i)}{\leq} \Qhat_h^t(s,\pi_t(s) ) - \Qstar_h(s,a) \\
%     &= \Phat_t(\cdot | s, \pi_t(s) )^\top \Vhat_{h+1}^t - \Phat_t(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} +   \Phat_t(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} - \Pstar(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} \\
%     &\leq \Phat_t(\cdot | s, \pi_t(s) )^\top \Vhat_{h+1}^t  - 
% \end{align*}
% Inequality $(i)$ holds because of optimism of $\Qhat_h^t(s,\pi_\star(s) )$. 





\end{proof}








\section{Supporting Results for Section~\ref{section::prunning_state_space}}

A consequence of Lemma~\ref{lemma::fixed_f_bound}, and Corollary~\ref{corollary::variance_bonus_domination},

\begin{corollary}\label{corollary::empirical_model_vs_v_tilde_bond}

Fix $\delta\in (0,1)$, $\forall t\in [1,2,\dots T],s\in \Scal,a\in \Acal,h\in [0,1,\dots,H-1]$, consider $\forall~ \Vtilde_h:\Scal \mapsto [0,H]$ with probability at least $1-\delta$:

\begin{equation*}
    \abs{\Phat_t(\cdot|s,a)^\top \Vtilde_{h+1} - \Pstar(\cdot|s,a)^\top \Vtilde_{h+1}} \leq 16\sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }\left[\Vtilde^2_{h+1}(s') | s,a\right]  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta} }{ N_h^t(s,a) }} + \frac{12H}{N_h^t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta}.
\end{equation*}

\end{corollary}


And therefore, defining $\tilde{b}_h^t(s,a) = 16\beta\sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }\left[\Vtilde^2_{h+1}(s') | s,a\right]  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta} }{ N_h^t(s,a) }} + \frac{12\beta H}{N_h^t(s,a)}\ln \frac{ 2 |\Scal| |\Acal|t}{\delta}$, 
% \aldo{the value of $\tilde{b}_h^t(s,a)$ is effectively the same as $b_h^t(s,a)$ (up to a scaling of the low order term).}

\begin{corollary}\label{corollary::upper_bound_empirical_Q_with_Qtildeu}
With probability at least $1-2\delta$ the empirical $Q$ function of state action pair $(s,a)$ satisfies,
\begin{equation*}
      \Qhat_h^t(s,a)  \leq r(s,a) + b_h^t(s,a) + \tilde{b}_h^t(s,a) + \beta \Pstar(\cdot|s,a)^\top \Vtilde_{h+1} := \Qtilde^u(s,a) +  b_h^t(s,a) +  \tilde{b}_h^t(s,a).
\end{equation*}
for all $s,a \in \Scal \times \Acal$ and for all $h \in [0, \cdots, H-1]$. 
\end{corollary}

\begin{proof}
By definition $\widehat Q_h^t(s,a) = r(s,a) + b_h^t(s,a) + \Phat^t(\cdot | s,a) \Vhat^t_{h+1}$, since $\Vhat^t_{h+1}$ is clipped above by $\beta \Vtilde_{h+1}$,
\begin{align*}
\widehat Q_h^t(s,a) &= r(s,a) + b_h^t(s,a) + \Phat^t(\cdot | s,a) \Vhat^t_{h+1} \\
&\leq r(s,a) + b_h^t(s,a) + \beta \Phat^t(\cdot | s,a) \Vtilde_{h+1}\\
&\leq r(s,a) + b_h^t(s,a) +  \tilde b^t_h(s,a) + \beta \Pstar(\cdot | s,a)^\top \Vtilde_{h+1}
\end{align*}
The last inequality follows by Corollary~\ref{corollary::empirical_model_vs_v_tilde_bond}. The result follows.


\end{proof}

The last corollary implies that once $b_h^t(s,a) + \tilde{b}_h^t(s,a) <  \Vstar(s) - \Qtilde^u(s,a)$ optimism guarantees that from that point on, action $a$ will never again be taken at state $s$. Indeed, since $\widehat{Q}_h^t(s,\pi_\star(s))$ is at least $\Vstar(s)$, action $a$ will be dominated by action $\pi_\star(s)$ from that point onwards. We make this intuition precise in the following Lemma.

\begin{lemma}\label{lemma::bounding_visitation_pseudosub}
With probability at least $1-2\delta$, the values of $N_t(s,a)$ for all $(s,a) \in \pseudosub_\Delta $ satisfy the bound,
\begin{equation*}
    N_t(s,a) \leq \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}
\end{equation*}
For all $t \in \mathbb{N}$. \aldo{Is this lemma used?}

\end{lemma}

\begin{proof}

Once $b_h^t(s,a) + \tilde{b}_h^t(s,a) <  \Vtilde(s) - \Qtilde^u(s,a)$ action $a$ will never be taken again at state $s$. The following bound holds for $b_h^t(s,a) + \tilde{b}_h^t(s,a)$,

\begin{align*}
    b_h^t(s,a) + \tilde{b}_h^t(s,a) &\leq 32 \beta \sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\Vtilde^2_{h+1}(s') | s,a ]  \ln\frac{ 2 |\Scal||\Acal|t}{\delta} }{ N_h^t(s,a) }}  +  \frac{24 \beta\max_{s'} \Vtilde_{h+1}(s')}{N_h^t(s,a)}\ln \frac{ 2 |\Scal||\Acal|t}{\delta} \\
    &\leq 32 \beta \max_{s} \Vtilde_{h+1}(s) \sqrt{\frac{\ln\frac{ 2 |\Scal||\Acal|t}{\delta}}{N_h^t(s,a)} } + \frac{24\beta\max_{s'} \Vtilde_{h+1}(s')}{N_h^t(s,a)}\ln \frac{ 2 |\Scal||\Acal|t}{\delta} 
\end{align*}

Assume $(s,a) \in \pseudosub_\Delta$. When 
\begin{equation*}
    N_h^t(s,a) > \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}
\end{equation*}
we get
\begin{equation}\label{equation::bounding_bonus_terms}
    b_h^t(s,a) + \tilde{b}_h^t(s,a) < \Delta \leq \Vstar(s) - \Qtilde^u(s,a) .
\end{equation}

The result follows because as soon as $b_h^t(s,a) + \tilde{b}_h^t(s,a) < \Delta$ holds, the optimism guarantees that from that point on action $a$ will never again be taken at state $s$. Indeed, let $\pi^\star(s)$ be the optimal action at state $s$,
\begin{equation*}
    \Qhat_h^t(s,\pi^\star(s) ) \geq \Qstar(s,\pi^\star(s)) = \Vstar(s) \geq \Qtilde^u(s,a) + \Delta 
\end{equation*}
Where the last inequality holds because by definition $(s,a) \in \pseudosub_\Delta$.

Plugging in the bound of Corollary~\ref{corollary::upper_bound_empirical_Q_with_Qtildeu}, and invoking inequality~\ref{equation::bounding_bonus_terms},

\begin{equation*}
     \Qhat_h^t(s,\pi^\star(s) ) \geq   \Qtilde^u(s,a) + \Delta  > \Qtilde^u(s,a) +  b_h^t(s,a) + \tilde{b}_h^t(s,a) \geq    \Qhat_h^t(s,a) .
\end{equation*}

implying action $a$ will not be selected by the greedy policy induced by the empirical $Q$ function $\Qhat_h^t$. This finalizes the result. 
\end{proof}

% \subsection{Proof of Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub}}\label{appendix::proof_lemma_upper_bound_visitation}

% \maxvisitationpseudosub
% SZ: I changed this restatable so that the hyperlink of the theorem in the main text is not pointing a theorem in the appendix


\begin{restatable}[Maximum Visitation of PseudoSuboptimal Pairs]{lemma}{maxvisitationpseudosub}\label{lemma::upper_bounding_sum_visitation_pseudosub-appendix}

With probability at least $1-2\delta$, the number of episodes whose sample trajectories contain a state from $\pathpseudosub_\Delta$ is upper bounded by,
\begin{align*}
   \sum_{t=1}^T \mathbf{1}( \tau_t \cap \left(\pathpseudosub_\Delta \cup \pseudosub_\Delta\right) \neq \emptyset) \leq
   |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \Vtilde^2 \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} 
\end{align*}
and
\begin{equation*}
    \sum_{(s,a) \in  \left (\left\{\pathpseudosub_\Delta \times \Acal \right \}\cup \pseudosub_\Delta\right)} N_T(s,a) \leq H \times |\boundarypseudosub_\Delta |\times \frac{8192 \beta^2 \times \Vtilde^2 \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}
\end{equation*}
%\aldo{This lemma can be written as instead intersections with $\pathpseudosub_\Delta \cup \pseudosub_\Delta$. It would be preferable to do so.}

\end{restatable}



% \begin{lemma}[Maximum Visitation of PseudoSuboptimal Pairs ]{lemma}{maxvisitationpseudosub}\label{lemma::upper_bounding_sum_visitation_pseudosub-appendix}

% With probability at least $1-2\delta$, the number of episodes whose sample trajectories contain a state from $\pathpseudosub_\Delta$ is upper bounded by,
% \begin{align*}
%   \sum_{t=1}^T \mathbf{1}( \tau_t \cap \left(\pathpseudosub_\Delta \cup \pseudosub_\Delta\right) \neq \emptyset) \leq
%   |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \Vtilde^2 \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} 
% \end{align*}
% and
% \begin{equation*}
%     \sum_{(s,a) \in  \left(\pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right)} N_T(s,a) \leq H \times |\boundarypseudosub_\Delta |\times \frac{8192 \beta^2 \times \Vtilde^2 \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}
% \end{equation*}
% %\aldo{This lemma can be written as instead intersections with $\pathpseudosub_\Delta \cup \pseudosub_\Delta$. It would be preferable to do so.}

% \end{lemma}




\begin{proof}

Let $\tau_t$ be the trajectory sampled by our algorithm at time $t$. Notice that whenever $\tau_t \cap \pathpseudosub_\Delta \neq \emptyset$, there must be a state action pair in $\tau_t$ (occurring previous to the state in $\tau_t$ that lies in  $\pathpseudosub_\Delta$ ) that is in $\boundarypseudosub_\Delta$, namely the first state-action pair belonging to $\pseudosub_\Delta$ in $\tau_t$. We obtain,

\begin{equation*}
    \sum_{t=1}^T \mathbf{1}( \tau_t \cap \left(\pathpseudosub_\Delta \cup \pseudosub_\Delta\right) \neq \emptyset ) \leq \sum_{t=1}^T \mathbf{1}( \tau_t \cap \boundarypseudosub_\Delta \neq \emptyset )
\end{equation*}

Lemma~\ref{lemma::bounding_visitation_pseudosub} implies that 
\begin{align*}
  \sum_{t=1}^T \mathbf{1}( \tau_t \cap \boundarypseudosub_\Delta \neq \emptyset )
  \leq&\;  \sum_{(s,a) \in \boundarypseudosub_\Delta} N_T(s,a)  \\
  \leq&\;|\boundarypseudosub_\Delta|\times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}
\end{align*}

Thus,
\begin{align*}
    &\sum_{t=1}^T \mathbf{1}( \tau_t \cap \left(\pathpseudosub_\Delta \cup \pseudosub_\Delta\right) \neq \emptyset )\qquad\\
    \leq &\; |\boundarypseudosub_\Delta|\times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}.
\end{align*}

Finalizing the proof of the first bullet. To prove the second bullet, the following inequalities hold
\begin{align*}
    &\sum_{(s,a) \in \left(\pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right)} N_t(s,a)\\
    \leq &\; H  \sum_{i=1}^t \mathbf{1}( \tau_t \cap \left(\pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right) \neq \emptyset )  \\
    \leq &\; H \sum_{i=1}^t \mathbf{1}( \tau_t \cap \boundarypseudosub_\Delta \neq \emptyset ) \\
    \leq &\; H \sum_{(s,a) \in \boundarypseudosub_\Delta} N_t(s,a)\\
    \leq &\; H \times |\boundarypseudosub_\Delta|\times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| t}{\delta} }{\Delta^2}.
\end{align*}
The result follows.
\end{proof}

\subsection{Full Version of Theorem~\ref{theorem::main_result}} 

\begin{theorem}
With probability at least $1-3\delta$,
 \begin{align*}
      &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
      \leq&\;\min\Bigg(   64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \notag\\
      &+ \frac{5793 \beta^2 \left(\max_h \Vtildemax_h\right)^2 \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |\mathcal{U}| |\boundarypseudosub_\Delta| }  }{\Delta}  \\
      &\;\notag 48H|\Scal | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) +  \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right),\\
      &\;64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \\
      & \;+ \notag48H|\Scal \times \Acal \backslash \mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) + \notag\\
      &\;2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \Bigg)      
 \end{align*}
For all $\Delta > 0$ simultaneously.

\end{theorem}





\begin{proof}
Lemma~\ref{lemma::indicator_upper_bound_regret} implies, 
\begin{align*}
     \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    &\quad \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) +\\
    &\quad \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
\end{align*}

Set $\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$. In what follows we will use $\mathcal{U}$ to denote this set when convenient. Recall that as a consequence of Equation~\ref{equation::neighbors_restricted} for all state action pairs $(s, a) \in \Scal \backslash \mathcal{U}$, we have that $\neighbor(s,a) \subseteq \Scal \backslash \pathpseudosub_\Delta$. Therefore, the support of $\Pstar(\cdot | s,a )$ and $\Phat_t(\cdot | s,a) $ is contained in $\Scal \backslash \pathpseudosub_\Delta$ for $(s,a) \in  \Scal \backslash ( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$. Lemma~\ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} implies,
\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left(  b_h^t(s^t_h, a^t_h) +\left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)  \\
     \leq&\;\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U})\left(  32 \beta \cdot \sqrt{ \frac{ |\Scal|  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s_h^t,a_h^t) }[\Vtilde^2_{h+1}(s') | s_h^t,a_h^t]  \ln\frac{ 8 \Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_h^t(s_h^t,a_h^t) }} +  \frac{24\Vtildemax_{h+1}}{N_h^t(s_h^t,a_h^t)}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|t^3}{\delta} \right) \\
     \leq&\; 32\beta \max_{h} \Vtildemax \sqrt{ | \Scal| \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }\left(\sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \in \mathcal{U})}{\sqrt{N_h^t(s_h^t, a_h^t)}} \right)  \\
    &+24\max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \in \mathcal{U})}{N_h^t(s_h^t, a_h^t)} .
\end{align*}
and
\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \Scal \backslash \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
    \leq\;&\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \Bigg(32 \beta \cdot \sqrt{ \frac{ |\Scal \backslash \pathpseudosub_\Delta |  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s_h^t,a_h^t) }[\Vtilde^2_{h+1}(s') | s_h^t,a_h^t]  \ln\frac{ 8\Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_h^t(s_h^t,a_h^t) }} + \\
    &+\frac{24\Vtildemax_{h+1}}{N_h^t(s_h^t,a_h^t)}\ln \frac{8\Vtildemax_{h+1} |\Scal| |\Acal|t^3}{\delta} \Bigg)\\
    \leq &\;32\beta \max_{h} \Vtildemax_h \sqrt{|\Scal \backslash \pathpseudosub_\Delta | \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }\left(\sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U})}{\sqrt{N_h^t(s_h^t, a_h^t)}} \right)+  \\
    & + 24\max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U})}{N_h^t(s_h^t, a_h^t)} .
\end{align*}

By Lemma~\ref{lemma:inverse_counts_bounds}, 

\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta) \left(  b_h^t(s^t_h, a^t_h) +\left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
  \leq &\;64\beta \max_{h} \Vtildemax_h \sqrt{ | \Scal| \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} } \times   \sqrt{H|\mathcal{U}|\sum_{(s,a) \in \mathcal{U}} \sum_{h=1}^{H} N_h^T(s,a)}  \\
  &\;+48H|\mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta}  \log(T+1)  \\
  \leq&\; \frac{5793 \beta^2 \left(\max_h \Vtildemax_h\right)^2 \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |\mathcal{U}| |\boundarypseudosub_\Delta| }  }{\Delta} \\
  &\;+48H|\mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1). 
\end{align*}
Where the last inequality follows from Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix} and where remember $\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$.

Similarly, Lemmas~\ref{lemma:inverse_squareroot_bounds} and~\ref{lemma:inverse_counts_bounds} imply,
\begin{equation}
     \label{equation::upper_bound_indicator_bonus_and_errors_s_minus_pathpseudosub}
     \begin{split}
         &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \Scal \backslash \left(\pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right)) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
      \leq \notag&\;64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal  \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \\
  &\;+ \notag 48H|\Scal \times \Acal \backslash \mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)
     \end{split}
\end{equation}
Combining these results we obtain,
\begin{equation}
\label{equation::upper_bound_regret_one}\begin{split}
      &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
      \leq&\;64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \\
      &\;+ \notag\frac{5793 \beta^2 \left(\max_h \Vtildemax_h\right)^2 \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |\mathcal{U}| |\boundarypseudosub_\Delta| }  }{\Delta}\\
      &\;+ \notag 48H|\Scal | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) +  \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
      \end{split}
 \end{equation}
We can also derive an almost $\Scal$-dependence free bound (with only a mild $\log(|\Scal|)$ dependence) at the cost of a quadratic dependence on the inverse $\frac{1}{\Delta}$. Lemma~\ref{lemma::indicator_upper_bound_regret} implies,


\begin{align*}
     &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
     \leq &\sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
    &\;+ \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
    \stackrel{(i)}{\leq}& \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)\\
    &\;+ \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
    \stackrel{(ii)}{\leq}&\;  \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    &\quad 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right).
    \end{align*}

Where inequality $(i)$ follows directly from the definition and inequality $(ii)$ from Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix}. Plugging in the inequality in Equation~\ref{equation::upper_bound_indicator_bonus_and_errors_s_minus_pathpseudosub}, we conclude,

\begin{equation}
    \label{equation::upper_bound_regret_two}
    \begin{split}
        &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
    \leq&\; 64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} } \\
  &\;\notag+ 48H|\Scal \times \Acal \backslash \mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)\\
  &\; +\notag 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right).
    \end{split}
\end{equation}
Since the two upper bounds~\ref{equation::upper_bound_regret_one} and~\ref{equation::upper_bound_regret_two} hold simultaneously, this concludes the proof. Where remember $\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$.


Interestingly, the upper bound~\ref{equation::upper_bound_regret_two} has only a logarithmic dependence on the size of the state space.


\end{proof}




\aldo{More refined result}

We start by proving a version of Lemma ~7.7 from~\cite{agarwal2019reinforcement}. 


\begin{lemma}\label{lemma::lem_7_7_theory_book}
With probability at least $1-\delta$ for all $h\in [H], t \in [T], s \in \Scal,a \in \Acal $ and all $f : \Scal \rightarrow \mathbb{R}$ such that $f_h(s) \in [ \Vtilde_h, \beta \Vtilde_h]$ we have,

\begin{equation*}
    \left| \left( \Phat_t(\cdot, s,a) - \Pstar(\cdot | s,a) \right)^\top f  \right| \leq \frac{\mathbb{E}_{s' \sim \Pstar_h(\cdot | s,a)}\left[ f(s') \right]}{H} +  \min\left(\frac{3H^2 | \mathrm{support}( \Pstar(\cdot |s,a) )|  }{N_h^t(s,a)} \ln\frac{\Vstarmax|\Scal||\Acal|t^3}{\delta}, \Vstarmax \right)
\end{equation*}




\end{lemma}


\begin{lemma}\label{lemma::lem_7_10_theory_book}
For all $t \in [1, \cdots T]$ we have,
\begin{align*}
    \Vstar(s_0) - V^{\pi_t}(s_0) = \Ocal\left(  \mathbb{E}_{\tau \sim \mathbb{P}^{\pi_t}} \left[ \sum_{h=1}^{H}  b_h^t(s_h^t, a_h^t) + \xi_h^t(a_h^t, s_h^t)  \right] \right)
\end{align*}
Where $\xi_h^t(a, s) = \min\left(\frac{2H^2 | \mathrm{support}( \Pstar(\cdot |s,a) )|  }{N_h^t(s,a)} \ln\frac{\Vstarmax|\Scal||\Acal|t^3}{\delta}, \Vstarmax \right)$. 
\end{lemma}

\begin{proof}
This lemma corresponds to lemma 7.10 in~\cite{agarwal2019reinforcement}. The proof is exactly the same, except that instead of using a uniform bound for the support of the distribution $\Pstar(\cdot |s,a)$ from Lemma 7.7. we use a support dependent version as in Lemma~\ref{lemma::lem_7_7_theory_book}.
\end{proof}



\begin{theorem}\label{theorem::refined_main_theorem}
With probability at least $1-3\delta$,
 \begin{align*}
      &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
      \leq&\;\min\Bigg(   64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \notag\\
      &+ \frac{5793 \beta^2 \left(\max_h \Vtildemax_h\right)^2 \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |\mathcal{U}| |\boundarypseudosub_\Delta| }  }{\Delta}  \\
      &\;\notag 48H|\Scal | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) +  \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right),\\
      &\;64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \\
      & \;+ \notag48H|\Scal \times \Acal \backslash \mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) + \notag\\
      &\;2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \Bigg)      
 \end{align*}
For all $\Delta > 0$ simultaneously.

\end{theorem}


\begin{proof}

Let $\mathcal{U} = \left(\pathpseudosub_\Delta \times \Acal \right)\cup \pseudosub_\Delta $. Lemma~\ref{lemma::lem_7_10_theory_book} implies, 

\begin{align*}
\sum_{t=1}^T \Vstar(s_0) - V^{\pi_t}(s_0) &= \Ocal\left(  \sum_{t=1}^T \mathbb{E}_{\tau \sim \mathbb{P}^{\pi_t}} \left[ \sum_{h=1}^{H}  b_h^t(s_h^t, a_h^t) + \xi_h^t(a_h^t, s_h^t)  \right] \right) \\
&=\underbrace{ \Ocal\left(  \sum_{t=1}^T \mathbb{E}_{\tau \sim \mathbb{P}^{\pi_t}} \left[ \sum_{h=1}^{H}  \mathbf{1}((s_h^t, a_h^t) \in \mathcal{U}) \left(b_h^t(s_h^t, a_h^t) + \xi_h^t(a_h^t, s_h^t)  \right)\right] \right) }_{\mathrm{I}}+\\
&\quad \underbrace{ \Ocal\left(  \sum_{t=1}^T \mathbb{E}_{\tau \sim \mathbb{P}^{\pi_t}} \left[ \sum_{h=1}^{H}  \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U}) \left(b_h^t(s_h^t, a_h^t) + \xi_h^t(a_h^t, s_h^t)  \right)\right] \right)}_{\mathrm{II}}
\end{align*}

We proceed to bound $\mathrm{I}$ and $\mathrm{II}$ independently. Our objective will be to derive a bound without dependence on the size of $\Scal$ (or at most logarithmic dependence on it) \aldo{revise this claim}. 

Recall that as a result of Equation~\ref{equation::neighbors_restricted}, the support of the dynamics for all $(s,a) \in. $ $|\mathrm{support}(\Pstar(\cdot |s,a)) | \leq | S\backslash \pathpseudosub_\Delta|$. 




Lemma~\ref{lemma::indicator_upper_bound_regret_refined_version} implies, 








\aldo{Old proof below}





Lemma~\ref{lemma::indicator_upper_bound_regret} implies, 







\begin{align*}
     \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    &\quad \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) +\\
    &\quad \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
\end{align*}

Set $\mathcal{U} = \left(\pathpseudosub_\Delta \times \Acal \right)\cup \pseudosub_\Delta$. In what follows we will use $\mathcal{U}$ to denote this set when convenient. Recall that as a consequence of Equation~\ref{equation::neighbors_restricted} for all state action pairs $(s, a) \in \Scal \backslash \mathcal{U}$, we have that $\neighbor(s,a) \subseteq \Scal \backslash \pathpseudosub_\Delta$. Therefore, the support of $\Pstar(\cdot | s,a )$ and $\Phat_t(\cdot | s,a) $ is contained in $\Scal \backslash \pathpseudosub_\Delta$ for $(s,a) \in  \Scal \backslash ( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$. Lemma~\ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} implies,
\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left(  b_h^t(s^t_h, a^t_h) +\left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)  \\
     \leq&\;\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U})\left(  32 \beta \cdot \sqrt{ \frac{ |\Scal|  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s_h^t,a_h^t) }[\Vtilde^2_{h+1}(s') | s_h^t,a_h^t]  \ln\frac{ 8 \Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_h^t(s_h^t,a_h^t) }} +  \frac{24\Vtildemax_{h+1}}{N_h^t(s_h^t,a_h^t)}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|t^3}{\delta} \right) \\
     \leq&\; 32\beta \max_{h} \Vtildemax \sqrt{ | \Scal| \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }\left(\sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \in \mathcal{U})}{\sqrt{N_h^t(s_h^t, a_h^t)}} \right)  \\
    &+24\max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \in \mathcal{U})}{N_h^t(s_h^t, a_h^t)} .
\end{align*}
and
\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \Scal \backslash \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
    \leq\;&\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \Bigg(32 \beta \cdot \sqrt{ \frac{ |\Scal \backslash \pathpseudosub_\Delta |  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s_h^t,a_h^t) }[\Vtilde^2_{h+1}(s') | s_h^t,a_h^t]  \ln\frac{ 8\Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_h^t(s_h^t,a_h^t) }} + \\
    &+\frac{24\Vtildemax_{h+1}}{N_h^t(s_h^t,a_h^t)}\ln \frac{8\Vtildemax_{h+1} |\Scal| |\Acal|t^3}{\delta} \Bigg)\\
    \leq &\;32\beta \max_{h} \Vtildemax_h \sqrt{|\Scal \backslash \pathpseudosub_\Delta | \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }\left(\sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U})}{\sqrt{N_h^t(s_h^t, a_h^t)}} \right)+  \\
    & + 24\max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U})}{N_h^t(s_h^t, a_h^t)} .
\end{align*}

By Lemma~\ref{lemma:inverse_counts_bounds}, \aldo{This lemma is the one that can be used to sum $\sum_{s,a} \frac{1}{\sqrt{N(s,a)}}$} 

\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left(  b_h^t(s^t_h, a^t_h) +\left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
  \leq &\;64\beta \max_{h} \Vtildemax_h \sqrt{ | \Scal| \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} } \times   \sqrt{H|\mathcal{U}|\sum_{(s,a) \in \mathcal{U}} \sum_{h=1}^{H} N_h^T(s,a)}  \\
  &\;+48H|\mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta}  \log(T+1)  \\
  \leq&\; \frac{5793 \beta^2 \left(\max_h \Vtildemax_h\right)^2 \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |\mathcal{U}| |\boundarypseudosub_\Delta| }  }{\Delta} \\
  &\;+48H|\mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1). 
\end{align*}
Where the last inequality follows from Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix} and where remember $\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$.

Similarly, Lemmas~\ref{lemma:inverse_squareroot_bounds} and~\ref{lemma:inverse_counts_bounds} imply,
\begin{equation}
     \label{equation::upper_bound_indicator_bonus_and_errors_s_minus_pathpseudosub}
     \begin{split}
         &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \Scal \backslash \left(\pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right)) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
      \leq \notag&\;64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal  \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \\
  &\;+ \notag 48H|\Scal \times \Acal \backslash \mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)
     \end{split}
\end{equation}
Combining these results we obtain,
\begin{equation}
\label{equation::upper_bound_regret_one}\begin{split}
      &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
      \leq&\;64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} }  \\
      &\;+ \notag\frac{5793 \beta^2 \left(\max_h \Vtildemax_h\right)^2 \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |\mathcal{U}| |\boundarypseudosub_\Delta| }  }{\Delta}\\
      &\;+ \notag 48H|\Scal | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) +  \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
      \end{split}
 \end{equation}
We can also derive an almost $\Scal$-dependence free bound (with only a mild $\log(|\Scal|)$ dependence) at the cost of a quadratic dependence on the inverse $\frac{1}{\Delta}$. Lemma~\ref{lemma::indicator_upper_bound_regret} implies,


\begin{align*}
     &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
     \leq &\sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
    &\;+ \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
    \stackrel{(i)}{\leq}& \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)\\
    &\;+ \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
    \stackrel{(ii)}{\leq}&\;  \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    &\quad 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right).
    \end{align*}

Where inequality $(i)$ follows directly from the definition and inequality $(ii)$ from Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix}. Plugging in the inequality in Equation~\ref{equation::upper_bound_indicator_bonus_and_errors_s_minus_pathpseudosub}, we conclude,

\begin{equation}
    \label{equation::upper_bound_regret_two}
    \begin{split}
        &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
    \leq&\; 64 H \beta \max_{h} \Vtildemax_h \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | |\Scal \times \Acal \backslash \mathcal{U}| T \ln\frac{ 8 \max_h \Vtildemax_{h} |\Scal| |\Acal| T^3}{\delta} } \\
  &\;\notag+ 48H|\Scal \times \Acal \backslash \mathcal{U} | \max_h \Vtildemax_{h}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)\\
  &\; +\notag 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \max_{s', h'} \Vtilde^2_{h'}(s') \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right).
    \end{split}
\end{equation}
Since the two upper bounds~\ref{equation::upper_bound_regret_one} and~\ref{equation::upper_bound_regret_two} hold simultaneously, this concludes the proof. Where remember $\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$.


Interestingly, the upper bound~\ref{equation::upper_bound_regret_two} has only a logarithmic dependence on the size of the state space.


\end{proof}







Thus we have the following simplified version of our results. Dropping all lower order terms from the result above,

\begin{corollary}
With probability at least $1-3\delta$,
\begin{align*}
\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) &= \Ocal\Bigg( \min_{\Delta}\Bigg(  H\beta \Vtildemax | \Scal \backslash \pathpseudosub_\Delta| \sqrt{ |\Acal| T \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} } +  \\
&\quad   \beta^2 \left(\Vtildemax\right)^2 \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} H^{1/2} \min \left( \frac{   |\Scal|^{3/2}|\Acal|  }{\Delta}, \frac{H^{3/2}|\boundarypseudosub_\Delta| }{\Delta^2}     \right)   \Bigg).
\end{align*}

\end{corollary}
 
$\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$




% \section{Sharper Theoretical Analysis}


% Let's start by considerting the following refinement to the upper bound of Equation~\ref{equation::simulation_optimism}. 

% \begin{align}
%     \sum_{t=1}^T \Vstar(s_0) - V^{\pi_t}(s_0) &\leq \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right] \notag\\
%     &\leq \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} -\Vstar_{h+1} \right)\right] + \notag\\
%     &\quad \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H  \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vstar_{h+1} \right]  \label{equation::simulation_optimism_refined} .
% \end{align}

% We have the following sharpened version of Lemma~\ref{lemma::indicator_upper_bound_regret}.



% \begin{lemma}\label{lemma::indicator_upper_bound_regret_sharpened}
% Let $\mathcal{U} \subseteq \Scal \times \Acal$ be an arbitrary subset of $\Scal \times \Acal$. With probability at least $1-\delta$,

% \begin{align*}
%     \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq \sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)+ \\
%     &\quad \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
%     &\leq \sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) \right)+ \\
%     &\quad \sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot  \Vstar_{h+1} \right)\\
%     &\quad \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
% \end{align*}
% And
% \begin{align*}
%     \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right)\right) + \\
%     &\quad \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left(  \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot  \Vstar_{h+1}\right) +\\
%     &\quad \sum_{t=1}^t\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
% \end{align*}
% % \aldo{Some of the $H$ dependence here can probably be turned into a $\Vtildemax$}

% % \textbf{Note:} An anytime bound is also possible. \aldo{consider changing this result to be anytime.}
% \end{lemma}

% \begin{proof}


% This follows immediately from Lemma~\ref{lemma::indicator_upper_bound_regret}. 


% \end{proof}




% By Lemma~\ref{} 

==> texs/supporting_technical_lemmas.tex <==
\section{Supporting Technical Lemmas}

\begin{lemma}[Anytime Hoeffding Inequality~\citep{pacchiano2020regret}]\label{lemma::anytime_hoeffding} Let $\{ Y_\ell\}_{\ell=1}^\infty$ be a martingale difference sequence such that $Y_\ell$ is $Y_\ell \in [a_\ell, b_\ell]$ almost surely for some constants $a_\ell, b_\ell$ almost surely for all $\ell = 1, \cdots, t$. then 

\begin{equation*}
      \sum_{\ell=1}^t Y_\ell \leq  2\sqrt{\sum_{\ell=1}^t (b_\ell-a_\ell)^2 \ln\left(\frac{12t^2}{\widetilde{\delta}}\right)} 
\end{equation*}
with probability at least $1-\widetilde{\delta}$ for all $t \in \mathbb{N}$ simultaneously.
\end{lemma}

\begin{lemma}[Freedman Bounded RVs - unsimplified~\citep{freedman1975tail,azar2017minimax}]\label{lemma:simplified_freedman}
Suppose $\{ X_t \}_{t=1}^\infty$ is a martingale difference sequence with $| X_t | \leq b$. Let 
\begin{equation*}
    \mathrm{Var}_\ell(X_\ell) = \mathrm{Var}( X_\ell | X_1, \cdots, X_{\ell-1})
\end{equation*}
Let $V_t = \sum_{\ell=1}^t \mathrm{Var}_\ell(X_\ell)$ be the sum of conditional variances of $X_t$.  Then we have that for any $\widetilde{\delta} \in (0,1)$ and $t \in \mathbb{N}$
\begin{equation*}
    \mathbb{P}\left(  \sum_{\ell=1}^t X_\ell >    2\sqrt{V_t}A_t + 3b A_t^2 \right) \leq \widetilde{\delta}
\end{equation*}
Where $A_t = \sqrt{2 \ln \ln \left(2 \left(\max\left(\frac{V_t}{b^2} , 1\right)\right)\right) + \ln \frac{6}{\widetilde{\delta}}}$.
% \aldo{Write this Bernstein version using the exact same statement as the Empirical Bernstein below.}
\end{lemma}


\begin{lemma}[Empirical Bernstein Anytime, Theorem 4 of~\cite{maurer2009empirical}]\label{lemma::bernstein_anytime}
Let $\ell \geq 2$ and $\left\{Z_t\right\}_{t=1}^\ell$ be i.i.d. random variables with distribution $Z$ satisfying $|Z_t| \leq b$ for all $t \in [\ell]$ 
% \aldo{Check if the absolute value here is correct. We may instead need to use the assumptions in \cite{maurer2009empirical}. In any case we can always shift the whole random variable}. 
Let the sample variance be defined as,
\begin{equation*}
    \mathrm{Var}_\ell(Z) = \frac{1}{\ell(\ell-1)} \sum_{1 \leq i < j \leq \ell} (Z_i - Z_j)^2
\end{equation*}
With probability at least $1-\delta$,
\begin{equation*}
    \mathbb{E}[ Z] - \frac{1}{\ell} \sum_{i=1}^\ell Z_i \leq \sqrt{\frac{4  \mathrm{Var}_\ell(Z) \ln \frac{4\ell^2}{\delta} }{ \ell} } + \frac{7 b \ln \frac{4\ell^2}{\delta}}{3(\ell-1)}
\end{equation*}
for all $\ell \in [\mathbb{N}]$
\end{lemma}
% \simon{The result from Theorem 4 of~\cite{maurer2009empirical} assumes $\mb Z\in [0,1]$, and show the inequality in the form of
% \begin{equation*}
%     \mathbb{E}[ Z] - \frac{1}{\ell} \sum_{i=1}^\ell Z_i \leq \sqrt{\frac{2 \mathrm{Var}_\ell(Z) \ln \frac{2}{\delta} }{ \ell} } + \frac{7 b \ln \frac{2}{\delta}}{3(\ell-1)}
% \end{equation*}
% but here we assume the $\abs{Z_i}\leq b$. The results in~\cite{maurer2009empirical} only apply half of the result to $[0,1]$ (I guess they make the assumption to control the cardinality of the hypothesis class $|\mc{F}|$), so that $|\mc F|$ does not scale with the dimension.}


\begin{lemma}[Lemma 7.5 of \cite{agarwal2019reinforcement}] 
\label{lemma:inverse_squareroot_bounds}
Consider arbitrary $T$ sequence of trajectories $\tau_t = \{s_h^t,a_h^t\}_{h=1}^{H}$, for $t = 0,1,\dots, T$. We have
\begin{equation}
    \sum_{t=1}^{T}\sum_{h=1}^{H}\frac{\mathbf{1}((s_h^t, a_h^t) \in \mathcal{U})  }{\sqrt{N_h^t(s_h^t,a_h^t)}}\leq 2\sqrt{H|\mathcal{U}|\sum_{(s,a) \in \mathcal{U}} \sum_{h=1}^{H} N_h^T(s,a)}  \leq 2H\sqrt{|\mathcal{U}|T}.
\end{equation}
Where $\mathcal{U} \subseteq \Scal \times \Acal$ is an arbitrary set of state action pairs. 
\end{lemma}
\begin{proof}
Consider swapping the order of summation
\begin{equation}
    \begin{split}
        &\sum_{t=1}^{T}\sum_{h=1}^{H}\frac{1}{\sqrt{N_h^t(s_h^t,a_h^t)}} = \sum_{h=1}^{H}\sum_{t=1}^{T}\frac{1}{\sqrt{N_h^t(s_h^t,a_h^t)}} = \sum_{(s,a)\in \mathcal{U}}\sum_{h=1}^{H}\sum_{i=1}^{N_h^T(s,a)}\frac{1}{\sqrt{i}}\\
        &\leq 2\sum_{(s,a)\in \mathcal{U}}\sum_{h=1}^{H}\sqrt{N_h^T(s,a)}\leq 2\sqrt{H|\mathcal{U}| \sum_{h=1}^{H}\sum_{(s,a) \in \mathcal{U}} N_h^T(s,a)} \leq 2H\sqrt{|\mathcal{U}|T},
    \end{split}
\end{equation}

where the first inequality use the fact that $\sum_{i=1}^N1/\sqrt{i}\leq 2\sqrt{N}$ and the second inequality holds due to Cauchy-Schwarz inequality. 
\end{proof}


\begin{lemma}[Sum of inverse counts]\label{lemma:inverse_counts_bounds}
Consider arbitrary $T$ sequence of trajectories $\tau_t = \{s_h^t,a_h^t\}_{h=1}^{H}$, for $t = 0,1,\dots, T$. We have
\begin{equation}
    \sum_{t=1}^{T}\sum_{h=1}^{H}\frac{\mathbf{1}((s_h^t, a_h^t) \in \mathcal{U})  }{N_h^t(s_h^t,a_h^t)}\leq 2|\mathcal{U}| H \log(T+1).
\end{equation}
Where $\mathcal{U} \subseteq \Scal \times \Acal$ is an arbitrary set of state action pairs. 
\end{lemma}
\begin{proof}
Consider swapping the order of summation
\begin{equation}
    \begin{split}
        &\sum_{t=1}^{T}\sum_{h=1}^{H}\frac{1}{{N_h^t(s_h^t,a_h^t)}} = \sum_{h=1}^{H}\sum_{t=1}^{T}\frac{1}{{N_h^t(s_h^t,a_h^t)}} = \sum_{(s,a)\in \mathcal{U}}\sum_{h=1}^{H}\sum_{i=1}^{N_h^T(s,a)}\frac{1}{{i}}\\
        &\leq 2\sum_{(s,a)\in \mathcal{U}}\sum_{h=1}^{H}\log\left(N_h^T(s,a)+1\right)\leq 2|\mathcal{U}| H \log(T+1)
    \end{split}
\end{equation}

\end{proof}




==> texs/theoretical_analysis.tex <==
\section{Analyzing UCBVI-Shaped}
\label{sec:analysis}
\vspace{-0.5em}
% We consider an episodic Markov Decision process $\Mcal = (\Scal, \Acal, \Tcal, r, H)$ where $\Scal$ corresponds to the state space, $\Acal$ is the action space, $\Tcal$ is the transition operator, $r : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the reward function and $H$ is the problem horizon. 
 
% \begin{assumption}\label{assump::sandwich}
% We assume access to shaping `value function' estimators $\widetilde{V}_h: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ such that,
% \begin{equation}\label{equation::V_tilde_sandwich}
%   \Vtilde_h(s)  \leq \Vstar_h(s)  \leq \beta \Vtilde_h(s)
% \end{equation}
% For all $s \in \Scal$, $h \in [H]$ and for some $ \beta \geq 1$.
% \end{assumption}







% For simplicity we will also assume the rewards are deterministic and have support in $[0,1]$. This assumption is in no way limiting and can be easily removed at a cost of a $\Ocal(\sqrt{T})$ in our regret bounds. 

% \begin{assumption}\label{assump::rewards}
% We assume the rewards are nonnegative and contained in $[0,1]$,
% \begin{equation*}
% r(s,a) \in [0,1] \qquad \forall s, a \in \Scal\times \Acal.    
% \end{equation*}
% \end{assumption}




% We consider a sequential interaction between a learner and the MDP $\mathcal{M}$ occuring in rounds indexed by $t \in \mathbb{N}$. At the start of round $t$ the learner selects a policy $\pi_t$ that is used to gather a sample trajectory from $\mathcal{M}$. We measure the learner's performance up to round $T$ by,

% \begin{equation*}
% \mathrm{Regret}(T)=      \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) 
% \end{equation*}

%  Where $s_0$ is the initial state, $V^{\pi}(s_0)$ is the expected value of using policy $\pi$ and $\Vstar(s_0)$ is the expected value of the optimal policy. Our objective is to design an algorithm such that with high probability satisfies a sublinear regret guarantee for all $T \in \mathbb{N}$. We would also like to show the leading term in this regret upper bound to depend on the effective state space of $\mathcal{M}$ as measured by the quality of $\Vtilde$. 

In this section, we will derive our main result on the sample complexity of the UCBVI-Shaped algorithm, and along the way introduce pseudosuboptimal and path-pseudosuboptimal states as a tool for deriving bounds that depend only on the ``effective'' state space as determined by the provided reward shaping. We will first introduce some notation to use in our analysis. As described in the previous section, UCBVI-Shaped proceeds in rounds. At the beginning of round $t$, the learner has access to an empirical model $\Phat_t$ built from the data collected up to iteration $t-1$. 
The bonus terms we consider are built by taking the empirical second moment of $\Vtilde$. This is related to the definition of $\mathrm{bonus\_2}$ in~\citet{azar2017minimax}. Importantly, the empirical value functions $\Vhat^t_h$ are clipped above by $\beta \Vtilde_h$. \vspace{-0.4em}
\begin{equation}
    \label{eq::shaped_bonus}
    b_h^t(s,a) =16 \beta \sqrt{ \frac{ \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s,a) }[\Vtilde^2_{h+1}(s') | s,a ]  \ln\frac{ 2 |\Scal||\Acal|}{\delta} }{ N_h^t(s,a) }}  +  \frac{12\beta \Vtildemax }{N_h^t(s,a)}\ln \frac{ 2 |\Scal||\Acal|t}{\delta}
\end{equation}
Where $\Vtildemax_{h} = \max_{s'} \Vtilde_h(s')$ and $\Vtildemax = \max_{s', h'} \Vtilde_{h'}(s')$. \aldo{Is $\Vtildemax_h$ ever used?}\simon{should the second $N_h^t(s,a)$ be $N_h^t(s,a)$?}
% We use the notation $\tau_t$ to denote the sample trajectory collected by the learner at round $t$. Trajectory $\tau_t$ is the sequence of states, actions and rewards $\tau_t = \Big(s_0^t, a_0^t, r(s_0^t, a_0^t),\cdots, s_{H-1}^t, a_{H-1}^t, r(s_{H-1}^t, a_{H-1}^t), s_H \Big)$. 

Despite clipping and a modified bonus term, the $\Qhat$ and $\Vhat$ values of UCBVI-Shaped are optimistic:
\begin{lemma}[Optimism]
\label{lemma::optimism}
With probability at least $1-\delta$  we have 
\begin{equation}
    \Vhat_0^t(s_0)\geq \Vstar_0(s_0),\;\forall s_0\in \Scal; \qquad \text{and} \qquad  \Qhat_h^t(s,a) \geq \Qstar_h(s,a), \quad \forall (s,a) \in \Scal\times \Acal,
\end{equation}
for all $t \in \mathbb{N}$, where $\Vhat_h^t$ is computed via Algorithm~\ref{algo:ValueIterationProj}.
\end{lemma}
The proof of Lemma~\ref{lemma::optimism} can be found in Appendix~\ref{appendix::lemma_optimism_proof}. Optimism (Lemma~\ref{lemma::optimism}) and the simulation Lemma~\citep{agarwal2019reinforcement} implies that:\vspace{-0.5em}
\begin{equation}\label{equation::simulation_optimism}
    \begin{small}
    \Vstar(s_0) - V^{\pi_t}(s_0) \leq \Vhat_1^t(s
    _0) -V^{\pi_t}(s_0)   = \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right].
    \end{small}
\end{equation}
We now turn our attention to characterize the information contained in $\Vtilde$. 

% Since by Lemma~\ref{lemma::optimism} the empirical value functions $\Vhat_h^t$ are optimistic, when $\mathcal{E}_{\mathrm{opt}}$ holds \aldo{what is $\mathcal{E}_{\mathrm{opt}}$?}, the simulation lemma implies that,
% \begin{equation*}
%     \Vstar(s_0 ) - V^{\pi_t}(s_0) \leq \Vhat_0^{t}(s_0) -V^{\pi_t}(s_0)  \leq \sum_{h=0}^{H-1} \mathbb{E}_{s_h, a_h \sim d^{\pi_t}} \left[ b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right]
% \end{equation*} 












\subsection{Pruning of the State Space}\label{section::prunning_state_space}
\vspace{-0.5em}
Consider the following ``surrogate'' Q functions, $\Qtilde_h^l, \Qtilde_h^u: \Scal \times \Acal \rightarrow \mathbb{R}$ induced by $\widetilde{V}$ via:
\begin{equation*}
    \Qtilde_h^l(s,a) = \mathbb{E}_{s' \sim \mathbb{P}(\cdot | s,a)}\left[ r(s,a) + \tilde{V}_{h+1}(s')\right], \qquad \widetilde Q_h^u(s,a) = \mathbb{E}_{s' \sim \mathbb{P}(\cdot | s,a)}\left[ r(s,a) + \beta \tilde{V}_{h+1}(s')\right].
\end{equation*}
By Assumption~\ref{assump::sandwich}, we can bound $Q^\star$ via $Q_h^\star(s,a) \in \left[\Qtilde_h^l(s,a),\Qtilde_h^u(s,a) \right]$. 
The basis of our results is the following observation. If an action $a$ satisfies $\Qtilde_h^u(s,a) < \Vstar_h(s)$ for state $s$, then $a$ is a suboptimal action for state $s$. Given a parameter $\Delta > 0$, we say that an action $a$ is $\Delta-$pseudosuboptimal\footnote{We add the qualifier pseudo to our name to distinguish between suboptimality as captured by our surrogate $Q$ values and true suboptimality between the true values of $Q_h^\star$. } for state $s$ if $\Vstar_h(s) \geq \Delta + \Qtilde_h^u(s,a)$. We denote the set of $\Delta-$pseudosuboptimal state action pairs as:
\begin{equation*}
    \pseudosub_\Delta = \{ (s,a) \in \Scal \times \Acal \text{ s.t. }   \Vstar_h(s) \geq \Delta + \Qtilde_h^u(s,a)\}.
\end{equation*}
The intuition we want to capture is that all states $\tilde s$ that can be accessed only through traversing a state action pair in $  \pseudosub_\Delta$, can be safely ignored. Because we can determine their suboptimality as soon as the state action pairs (or set of state action pairs) in $\pseudosub_\Delta$ that lead to $\tilde s$ are visited enough. 

% The intuition we want to capture is that all states $\tilde s$ that can be accessed only through traversing a state action pair in $  \pseudosub_\Delta$, can be safely ignored, because as soon as the state action pairs (or set of state action pairs) in $\pseudosub_\Delta$ that lead to $\tilde s$ are visited enough to determine their suboptimality.
% SZ: The sentence above has some grammar errors, I rephrased it a bit. Please correct me if my understanding is incorrect.

Now we define the set of $\Delta$-path-pseudosuboptimal states as the states that can be reached only by traversing a $\Delta-$pseudosuboptimal state action pair:
\begin{equation*}
    \pathpseudosub_\Delta = \{ s \in \Scal \text{ s.t. } \text{all feasible paths from initial states to $s$ intersect $\pseudosub_\Delta$} \}.
\end{equation*}
We will show that states in $\pathpseudosub_\Delta$ will not be explored by UCBVI-Shaped after a few iterations. Intuitively, this happens because the support of the state visitation distribution of the optimal policy does not contain any state in $\pathpseudosub_\Delta,\forall \Delta>0$ (or equivalently, $\mathrm{Support}( d^{\pi^\star}(s,a)   ) \cap  \pathpseudosub_\Delta = \emptyset, \forall \Delta > 0$). Hence, once the UCBVI-shaped identifies some sub-optimal state action pairs, the algorithm will not visit these state-action pairs again.

% To provide intuition of why this is the case, note the support of the optimal policy distribution does not contain any state in $\pathpseudosub_\Delta$ for all $\Delta > 0$, i.e.,  $\mathrm{Support}( d^{\pi^\star}(s,a)   ) \cap  \pathpseudosub_\Delta = \emptyset, \forall \Delta > 0$. 

For any state action pair $(s,a)$ define its set of neighboring states $\neighbor(s,a)$ as the set of states with nonzero probability in $\Pstar(\cdot | s,a)$. By definition of $\pathpseudosub_\Delta$, for all $(s, a) \in \Scal \backslash ( \left(\pathpseudosub_\Delta \times \Acal \right)\cup \pseudosub_\Delta)$, we have:
\begin{equation}\label{equation::neighbors_restricted}
    \neighbor(s,a) \subseteq \Scal \backslash \pathpseudosub_\Delta.
\end{equation}
In other words, the neighborhood of any state action pair $(s,a)$ whose state is not in $\pathpseudosub_\Delta$ and such that $(s,a)$ is not $\Delta-$pseudo-suboptimal, are not in $\pathpseudosub_\Delta$. We also introduce the notion of Boundary pseudosuboptimal state action pairs to capture the set of state action pairs that are $\Delta-$suboptimal but whose states are not in $\pathpseudosub_\Delta$. \vspace{-0.5em}
\begin{equation*}
     \boundarypseudosub_\Delta = \{ (s,a) \in \pseudosub_{\Delta} \text{ and } s \not\in \pathpseudosub_\Delta \}.  
\end{equation*}
Naturally, one of these states has to be traversed by any trajectory that contains any state in $\pathpseudosub_\Delta$.

Although we only use $\Qtilde^u$ in the definition of $\pseudosub_\Delta$, $\pathpseudosub_\Delta$, and $\boundarypseudosub_\Delta$, the size of these sets is modulated by the scale of $\beta$ and the width of the intervals $\left[\Qtilde^l(s,a),\Qtilde^u(s,a) \right]$. We will show that (in the notation of Theorem~\ref{theorem::informal_main}) $\Scal_{\mathrm{prunned}} \approx \Scal \backslash \pathpseudosub_\Delta$. With this notation, the formal version of our main results is stated as follows. 

\begin{theorem}\label{theorem::main_result}
With probability at least $1-3\delta$, the regret of UCBVI-Shaped is upper bounded by
\begin{small}
\begin{align*}
\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) =\;& \Ocal\Bigg( \min_{\Delta}\Bigg(  H\beta \Vtildemax | \Scal \backslash \pathpseudosub_\Delta| \sqrt{ |\Acal| T \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} } +  \\
&\beta^2 \left(\Vtildemax\right)^2 \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} H^{1/2} \min \left( \frac{   |\Scal|^{3/2}|\Acal|  }{\Delta}, \frac{H^{3/2}|\boundarypseudosub_\Delta| }{\Delta^2}     \right)   \Bigg).
\end{align*}
\end{small}
for all $T \in \mathbb{N}$.
\end{theorem}

Theorem~\ref{theorem::main_result} instantiates the desiderata of Theorem~\ref{theorem::informal_main}. Although this regret upper bound cannot be decomposed into a sum of two term as in Theorem~\ref{theorem::informal_main}. For any fixed $\Delta$, the regret upper bound does have two components, one where $\Scal_\mathrm{remain}$ can be identified with $| \Scal \backslash \pathpseudosub_\Delta|$ and a second one that scales logarithmically in $T$. In the next section we flesh out the steps in the proof of this result. The full argument can be found in Appendix~\ref{sec:supporting_lemmas}. The bonus scaling also allows us to ameliorate the horizon dependence of the upper bound. Instead of obtaining a $H^2$ dependence as the bound of theorem 7.1 in~\cite{agarwal2019reinforcement}, the first term depends on $\beta H\Vtildemax \leq \beta H \max_s \Vstar(s)$ \aldo{Is this what we want?}. 
% We expect the same result to hold for sharper analysis of UCBVI. 
% Although similar guarantees may be achieved by using an algorithm such as $\mathrm{EULER}$~\cite{zanette2019tighter}, we believe our result still carries merits as it shows that the knowledge of $\tilde{V}$ can be seamlessly incorporated into the bonus definition of existing algorithms to improve the horizon dependence of their bounds. 
Notice that the state dependence in the second term may be only be of order $\log(|\Scal|)$ if there is a $\Delta$ such that $|\boundarypseudosub_\Delta| \ll |\Scal|$  (albeit at the cost of a quadratic dependence on $1/\Delta^2$). Setting $\Delta$ to a value smaller than the minimum gap recovers the UCBVI regret upper bounds Theorem 7.1 in~\cite{agarwal2019reinforcement} showing Theorem~\ref{theorem::main_result} is a strict generalization.\vspace{-0.5em}

\subsection{Proof Intuitions and Sketch for Theorem~\ref{theorem::main_result}}
\vspace{-0.5em}
\paragraph{Improved Horizon Dependence.} An empirical Bernstein bound shows that adding a bonus scaling (up to low order terms) with $\Ocal\left(\sqrt{  \widehat{\mathrm{Var}}_{s' \sim \Phat_t(\cdot | s,a) }(\Vstar_{h+1}(s') | s,a)  \ln\frac{ 2 |\Scal| |\Acal| t}{\delta} / N_h^t(s,a) } \right) $ is sufficient to ensure optimism. Since $\Vstar$ is not known, this variance term can be substituted by the empirical second moment of $\beta\Vtilde_{h+1}$. Finally the scaling of these terms can be upper bounded by $\beta \Vtildemax$. Without knowledge of $\Vtilde$, achieving this scaling would prove more challenging, since the only proxy for $\Vstar_{h+1}$ available is $\Vhat_{h+1}^t$ or $H$ both of which may vastly overestimate it. \vspace{-0.5em}\vspace{-0.5em}

\paragraph{State Pruning.} The value function clipping mechanism ensures that $\mathbb{E}_{s' \sim \Phat_h(\cdot | s,a) } \left[  \Vhat^t_{h+1}(s') \right] \leq \beta \mathbb{E}_{s' \sim \Phat_h(\cdot | s,a) } \left[  \Vtilde_{h+1}(s') \right] $ and therefore the empirical gap between $\Qhat_h^t(s,a)$ and $\Vstar(s)$ is decreasing at a rate of at most $\Ocal\left( \beta\Vtildemax/\sqrt{N_h^t(s,a)} \right)$. Since optimism ensures that $\Qhat_h^t(s,\pi^\star(a)) \geq \Vstar(s)$, once $\Qhat(s,a)< \Vstar(s)$, action $a$ will not be pulled anymore. Thus for any $\Delta$, the number of times any state action pair in $\pseudosub_\Delta$ may be visited by UCBVI-Shaped is upper bounded by $\beta^2\left(\Vtildemax\right)^2/\Delta^2$. Since any visit to a state action pair in $\pathpseudosub_\Delta \times \mathcal{A} \cup \pseudosub_\Delta$ requires a visit to a state in $\boundarypseudosub_\Delta$, which allows us to bound the total number of visits to a state (or a trajectory containing such a state) in $\pathpseudosub_\Delta \times \mathcal{A} \cup \pseudosub_\Delta$ by $H|\boundarypseudosub_\Delta|\beta^2\left(\Vtildemax\right)^2/\Delta^2$.

Finally, we can split the regret decomposition of Eqn.~\ref{equation::simulation_optimism} into two sums, one over state action pairs in  $\mathcal{U} = \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta$ (or trajectories intersecting $\mathcal{U}$) and a second one over state action pairs in $\mathcal{U}^c$ (or trajectories without intersection with $\mathcal{U}$ ). We can then apply the upper bound on the visitation of state action pairs (or trajectories ) in $\pathpseudosub_\Delta \times \mathcal{A} \cup \pseudosub_\Delta$ to derive a regret upper bound over these states scaling with $1/\Delta$. Using the trajectory decomposition yields the term scaling with $1/\Delta^2$ (but having only logarithmic state dependence) in Theorem~\ref{theorem::main_result}. We handle the upper bound for the term summing over intersections with $\mathcal{U}^c$ by noting that Eqn.~\ref{equation::neighbors_restricted} implies the transition operators over state action pairs in $\mathcal{U}^c$ have support only over $\Scal \backslash \pathpseudosub_\Delta$. This implies the error terms$\left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}$ can be bounded by a factor depending on $|\Scal \backslash \pathpseudosub_\Delta|$ and not $|\Scal|$. Detailed proofs can be found in Appendix~\ref{sec:supporting_lemmas}. \vspace{-0.5em}


==> texs_copy/dprecated_lemmas.tex <==
The following Lemma provides us with a regret decomposition that will be important in the proof of Lemma~\ref{theorem::main_result},

\begin{lemma}\label{lemma::indicator_upper_bound_regret}
Let $\mathcal{U} \subseteq \Scal \times \Acal$ be an arbitrary subset of $\Scal \times \Acal$. With probability at least $1-\delta$,

\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  \leq \qquad \qquad \qquad \qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad \qquad  \qquad \qquad  \\
    \qquad \sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left(\Vhat_{h+1}^{\pi_t} -\Vstar_{h+1}\right)\right)+ \\
    \qquad  \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \qquad \qquad \qquad \qquad \qquad\qquad \qquad \quad
\end{align*}

And
\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  \leq  \qquad \qquad \qquad \qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad  \qquad \qquad \\
    \qquad \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \left( \Vhat_{h+1}^{\pi_t} - \Vstar_{h+1}\right) \right) + \\
    \qquad \sum_{t=1}^t\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \qquad \qquad \qquad \qquad \qquad\qquad \qquad 
\end{align*}
% \aldo{Some of the $H$ dependence here can probably be turned into a $\Vtildemax$}

% \textbf{Note:} An anytime bound is also possible. \aldo{consider changing this result to be anytime.}
\end{lemma}




\begin{proof}


First note that by the simulation lemma, optimism (see Equation~\ref{equation::simulation_optimism}) and by Hoeffding inequality. 

\begin{align*}
    \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) &\leq \sum_{t=1}^T \mathbb{E}_{\tau \sim \pi_t }\left[ \sum_{h=1}^H \paren{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}}  \right]\\
    &\leq \sum_{t=1}^T \sum_{h=1}^H \paren{b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}}  + \Ocal\left(H\sqrt{ TH \ln(T/\delta)   }     \right)
\end{align*}
with probability at least $1-\delta$. The inequality above is satisfied because
\begin{align*}
\abs{b_h^t(s_h, a_h) + \left( \Phat_t(\cdot | s_h, a_h) - \Pstar( \cdot | s_h, a_h) \right) \cdot \Vhat_{h+1}^{\pi_t}  }\leq 2H     
\end{align*}

We will now 



% \aldo{We now turn to bounding the trajectory based stuff}


% \aldo{this $H$ dependence can probably be traded with a $\max \Vtilde$ one}. 
Next notice that $\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t}   \leq 2H^2$ and therefore, 

\begin{align*}
    &\sum_{t=1}^T \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \\
    \leq&\;\sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}  = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)+  \sum_{t=1}^t \mathbf{1}(\tau_t \cap \mathcal{U} \neq \emptyset) 2H^2  
\end{align*}

Similarly, 
\begin{align*}
    &\sum_{t=1}^T \sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \\
    \leq&\;\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \sum_{t=1}^T\sum_{h=1}^H \mathbf{1}((s_h^t, a_h^t) \not\in \mathcal{U} )2 H
\end{align*}

The result follows.
% Finally, let's prove an upper bound for $\Qstar(s,\pi_\star(s)) - \Qstar(s,\pi_t(s))$. 

% \begin{align*}
%     \Qstar_h(s,\pi_\star(s) ) - \Qstar_h(s,\pi_t(s)) &\stackrel{(i)}{\leq} \Qhat_h^t(s,\pi_t(s) ) - \Qstar_h(s,a) \\
%     &= \Phat_t(\cdot | s, \pi_t(s) )^\top \Vhat_{h+1}^t - \Phat_t(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} +   \Phat_t(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} - \Pstar(\cdot | s, \pi_t(s) )^\top \Vstar_{h+1} \\
%     &\leq \Phat_t(\cdot | s, \pi_t(s) )^\top \Vhat_{h+1}^t  - 
% \end{align*}
% Inequality $(i)$ holds because of optimism of $\Qhat_h^t(s,\pi_\star(s) )$. 





\end{proof}



\subsection{Full Version of Theorem~\ref{theorem::main_result}} 

\begin{theorem}
With probability at least $1-3\delta$,
 \begin{align*}
      &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
      \leq&\;\min\Bigg(   64 H \beta \Vtildemax \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | | \mathcal{U}^{\mathrm{good}}| T \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} }   \notag\\
      &\;+ \frac{5793 \beta^2 \left( \Vtildemax\right)^2 \ln\frac{ 8  \Vtildemax |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |(\Scal \times \Acal) \backslash\mathcal{U}^{\mathrm{good}}| |\boundarypseudosub_\Delta| }  }{\Delta} \notag\\
      &\;+ \notag 96H|\Scal|^2|\Acal| \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1),\\
      &\;  64 H \beta \Vtildemax \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | | \mathcal{U}^{\mathrm{good}}| T \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} }\notag\\
  &\;+48H|\mathcal{U}^{\mathrm{good}} | |\Scal \backslash \pathpseudosub_\Delta | \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)\notag\\
  &\; + 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \left( \Vtildemax\right)^2 \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2}  \Bigg)      + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) 
 \end{align*}
Where $\mathcal{U}^{\mathrm{good}} = (\Scal \times \Acal )\backslash\left( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right)$. For all $\Delta > 0$ simultaneously.

\end{theorem}





\begin{proof}
Lemma~\ref{lemma::indicator_upper_bound_regret} implies, 
\begin{align*}
     \sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)  &\leq \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    &\quad \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) +\\
    &\quad \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right)
\end{align*}

Set $\mathcal{U}^{\mathrm{good}} = (\Scal \times \Acal )\backslash\left( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta\right)$ to be the set of 'good states'. In what follows we will use $\mathcal{U}^{\mathrm{good}}$ to denote this set when convenient. Recall that as a consequence of Equation~\ref{equation::neighbors_restricted} for all state action pairs $(s, a) \in \mathcal{U}^{\mathrm{good}}$, we have that $\neighbor(s,a) \subseteq \Scal \backslash \pathpseudosub_\Delta$. Therefore, the support of $\Pstar(\cdot | s,a )$ and $\Phat_t(\cdot | s,a) $ is contained in $\Scal \backslash \pathpseudosub_\Delta$ for $(s,a) \in \mathcal{U}^{\mathrm{good}} = ( \Scal \backslash ( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$. Lemma~\ref{lemma:ModelErrorEmpiricalBernsteinGeneralized} implies,
\begin{align}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in  \mathcal{U}^{\mathrm{good}}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \label{equation::supporting_equation_pairs_good}\\
    \leq\;&\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}^{\mathrm{good}}) \Bigg(32 \beta \cdot \sqrt{ \frac{  |\Scal \backslash \pathpseudosub_\Delta |  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s_h^t,a_h^t) }[\Vtilde^2_{h+1}(s') | s_h^t,a_h^t]  \ln\frac{ 8\Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_h^t(s_h^t,a_h^t) }} + \notag \\
    &+\frac{24\Vtildemax_{h+1} |\Scal \backslash \pathpseudosub_\Delta | }{N_h^t(s_h^t,a_h^t)}\ln \frac{8\Vtildemax_{h+1} |\Scal| |\Acal|t^3}{\delta} \Bigg)\notag\\
    \leq &\;32\beta \Vtildemax \sqrt{|\Scal \backslash \pathpseudosub_\Delta | \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} }\left(\sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}^{\mathrm{good}})}{\sqrt{N_h^t(s_h^t, a_h^t)}} \right)+  \notag\\
    & + 24 \Vtildemax |\Scal \backslash \pathpseudosub_\Delta |\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}^{\mathrm{good}})}{N_h^t(s_h^t, a_h^t)} .\notag
\end{align}
and
\begin{align}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}^{\mathrm{good}}) \left(  b_h^t(s^t_h, a^t_h) +\left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \label{equation::supporting_equation_pairs_good_complement} \\
     \leq&\;\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not\in  \mathcal{U}^{\mathrm{good}})\left(  32 \beta \cdot \sqrt{ \frac{ |\Scal|  \widehat{\mathbb{E}}_{s' \sim \Phat_t(\cdot | s_h^t,a_h^t) }[\Vtilde^2_{h+1}(s') | s_h^t,a_h^t]  \ln\frac{ 8 \Vtildemax_{h+1} |\Scal| |\Acal| t^3}{\delta} }{ N_h^t(s_h^t,a_h^t) }} +  \frac{24\Vtildemax_{h+1}|\Scal|}{N_h^t(s_h^t,a_h^t)}\ln \frac{8 \Vtildemax_{h+1}|\Scal| |\Acal|t^3}{\delta} \right) \notag\\
     \leq&\; 32\beta \Vtildemax \sqrt{ | \Scal| \ln\frac{ 8  \Vtildemax |\Scal| |\Acal| T^3}{\delta} }\left(\sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}^{\mathrm{good}})}{\sqrt{N_h^t(s_h^t, a_h^t)}} \right)  \notag\\
    &+24 \Vtildemax|\Scal|\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \sum_{t=1}^T \sum_{h=1}^H \frac{\mathbf{1}((s^t_h, a^t_h) \not\in \mathcal{U}^{\mathrm{good}})}{N_h^t(s_h^t, a_h^t)} .\notag
\end{align}
By Lemmas~\ref{lemma:inverse_squareroot_bounds} and~\ref{lemma:inverse_counts_bounds} equation~\ref{equation::supporting_equation_pairs_good} can be upper bounded by,
\begin{align}
     \label{equation::upper_bound_indicator_bonus_and_errors_s_minus_pathpseudosub}
         &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in \mathcal{U}^{\mathrm{good}}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
      \leq \notag&\;64 H \beta \Vtildemax \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | | \mathcal{U}^{\mathrm{good}}| T \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} } \notag \\
  &\;+ \notag 48H|\mathcal{U}^{\mathrm{good}} | |\Scal \backslash \pathpseudosub_\Delta | \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) \notag
\end{align}


Similarly by Lemmas~\ref{lemma:inverse_squareroot_bounds},~\ref{lemma:inverse_counts_bounds} and~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix} , we can upper bound the RHS of Equation~\ref{equation::supporting_equation_pairs_good_complement} as,
\begin{align*}
    &\sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \not \in \mathcal{U}^{\mathrm{good}}) \left(  b_h^t(s^t_h, a^t_h) +\left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
  \leq &\;64\beta  \Vtildemax \sqrt{ | \Scal| \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} } \times   \sqrt{H|(\Scal \times \Acal) \backslash \mathcal{U}^{\mathrm{good}}|\sum_{(s,a) \in (\Scal \times \Acal) \backslash\mathcal{U}^{\mathrm{good}}} \sum_{h=1}^{H} N_h^T(s,a)}  \\
  &\;+48H|(\Scal \times \Acal)  \backslash \mathcal{U}^{\mathrm{good}} |  \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta}  \log(T+1)  \\
  \leq&\; \frac{5793 \beta^2 \left( \Vtildemax\right)^2 \ln\frac{ 8  \Vtildemax |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |(\Scal \times \Acal) \backslash\mathcal{U}^{\mathrm{good}}| |\boundarypseudosub_\Delta| }  }{\Delta} \\
  &\;+\underbrace{48H|(\Scal \times \Acal) \backslash\mathcal{U}^{\mathrm{good}} | |\Scal|\Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)}_{\leq 48H|\Scal|^2|\Acal| \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1) }. 
\end{align*}
Where the last inequality follows from Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix} and where remember $\mathcal{U}^{\mathrm{good}} = (\Scal \times \Acal) \backslash (\pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$.

Combining these results we obtain,
\begin{align}
\label{equation::upper_bound_regret_one}
      &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
      \leq&\;64 H \beta \Vtildemax \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | | \mathcal{U}^{\mathrm{good}}| T \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} }   \notag\\
      &\;+ \frac{5793 \beta^2 \left( \Vtildemax\right)^2 \ln\frac{ 8  \Vtildemax |\Scal| |\Acal| T^3}{\delta} \sqrt{H |\Scal| |(\Scal \times \Acal) \backslash\mathcal{U}^{\mathrm{good}}| |\boundarypseudosub_\Delta| }  }{\Delta} \notag\\
      &\;+ \notag 96H|\Scal|^2|\Acal| \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)+  \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \notag
 \end{align}



%%%%%%%%%%%% HEEEEEREREREREEREE  %%%%%%%%%%%%%%%%



Now define $\mathcal{U}^{\mathrm{bad}} = \left(\left[\pathpseudosub_\Delta \times \Acal\right] \cup \pseudosub_\Delta\right)$ be the 'bad' state-action pairs. We can also derive an almost $\Scal$-dependence free bound (with only a mild $\log(|\Scal|)$ dependence) at the cost of a quadratic dependence on the inverse $\frac{1}{\Delta}$. Lemma~\ref{lemma::indicator_upper_bound_regret} implies,

\begin{align*}
     &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)\\
     \leq &\sum_{t=1}^T \mathbf{1}( \tau_t \cap \mathcal{U}^{\mathrm{bad}} = \emptyset ) \left(\sum_{h=1}^H b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) \\
    &\;+ \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U}^{\mathrm{bad}} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
    \stackrel{(i)}{\leq}& \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in (\Scal \times \Acal) \backslash \mathcal{U}^{\mathrm{bad}}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right)\\
    &\;+ \sum_{t=1}^T \mathbf{1}(\tau_t \cap \mathcal{U}^{\mathrm{bad}} \neq \emptyset) 2H^2  + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right) \\
    \stackrel{(ii)}{\leq}&\;  \sum_{t=1}^T  \sum_{h=1}^H \mathbf{1}((s^t_h, a^t_h) \in (\Scal \times \Acal) \backslash \mathcal{U}^{\mathrm{bad}}) \left( b_h^t(s^t_h, a^t_h) + \left( \Phat_t(\cdot | s^t_h, a^t_h) - \Pstar( \cdot | s^t_h, a^t_h) \right) \cdot \Vhat_{h+1}^{\pi_t} \right) + \\
    &\quad 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \left( \Vtildemax\right)^2 \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right).
    \end{align*}

Where inequality $(i)$ follows directly from the definition and inequality $(ii)$ from Lemma~\ref{lemma::upper_bounding_sum_visitation_pseudosub-appendix}. Plugging in the inequality in Equation~\ref{equation::upper_bound_indicator_bonus_and_errors_s_minus_pathpseudosub}, and using the fact that $\mathcal{U}^{\mathrm{good}} = (\Scal \times \Acal) \backslash \mathcal{U}^{\mathrm{bad}}$ we conclude,

\begin{align}
   % \begin{split}
        &\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0)   \label{equation::upper_bound_regret_two}\\
    \leq&\; 64 H \beta \Vtildemax \sqrt{  |\Scal \backslash \pathpseudosub_\Delta | | \mathcal{U}^{\mathrm{good}}| T \ln\frac{ 8 \Vtildemax |\Scal| |\Acal| T^3}{\delta} }\notag\\
  &\;+48H|\mathcal{U}^{\mathrm{good}} | |\Scal \backslash \pathpseudosub_\Delta | \Vtildemax\ln \frac{8 \Vtildemax|\Scal| |\Acal|T^3}{\delta} \cdot \log(T+1)\notag\\
  &\; + 2H^2 |\boundarypseudosub_\Delta| \times \frac{8192 \beta^2 \times \left( \Vtildemax\right)^2 \cdot \ln \frac{2 |\Scal||\Acal| T}{\delta} }{\Delta^2} + \Ocal\left( H\sqrt{TH\ln(T/\delta)} \right).\notag
%    \end{split}
\end{align}
Since the two upper bounds~\ref{equation::upper_bound_regret_one} and~\ref{equation::upper_bound_regret_two} hold simultaneously, this concludes the proof. Where remember $\mathcal{U} = (\Scal \times \Acal)\backslash( \pathpseudosub_\Delta \times \Acal \cup \pseudosub_\Delta)$.
  

Interestingly, the upper bound~\ref{equation::upper_bound_regret_two} has only a logarithmic dependence on the size of the state space.


\end{proof}











Thus we have the following simplified version of our results. Dropping all lower order terms from the result above,

\begin{corollary}
With probability at least $1-3\delta$,
\begin{align*}
\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) &= \Ocal\Bigg( \min_{\Delta}\Bigg(  H\beta \Vtildemax  | \Scal \backslash \pathpseudosub_\Delta|\sqrt{ |\Acal| T \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} } +  \\
&\quad   \beta^2 \left(\Vtildemax\right)^2 \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} H^{1/2} \min \left( \frac{   |\Scal|^{3/2}|\Acal|  }{\Delta}, \frac{H^{3/2}|\boundarypseudosub_\Delta| }{\Delta^2}     \right)   \Bigg).
\end{align*}

\end{corollary}
 



\begin{theorem}\label{theorem::main_result}
With probability at least $1-6\delta$, the regret of UCBVI-Shaped is upper bounded by

\begin{small}
\begin{align*}
\sum_{t=1}^T   \Vstar(s_0) - V^{\pi_t}(s_0) =\;& \Ocal\Bigg( \min_{\Delta}\Bigg(  H\beta \Vtildemax | \Scal \backslash \pathpseudosub_\Delta| \sqrt{ |\Acal| T \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} } +  \\
&\beta^2 \left(\Vtildemax\right)^2 \ln \frac{\Vtildemax |\Scal| |\Acal| T}{\delta} H^{1/2} \min \left( \frac{   |\Scal|^{3/2}|\Acal|  }{\Delta}, \frac{H^{3/2}|\boundarypseudosub_\Delta| }{\Delta^2}     \right)   \Bigg),
\end{align*}
\end{small}
for all $T \in \mathbb{N}$.
\end{theorem}
